Blades: A Unified Benchmark Suite for Byzantine Attacks and Defenses in Federated Learning

Federated learning (FL) facilitates distributed training across different IoT and edge devices, safeguarding the privacy of their data. The inherent distributed structure of FL introduces vulnerabilities, especially from adversarial devices aiming to skew local updates to their advantage. Despite the plethora of research focusing on Byzantine-resilient FL, the academic community has yet to establish a comprehensive benchmark suite, pivotal for impartial assessment and comparison of different techniques. This paper presents Blades, a scalable, extensible, and easily configurable benchmark suite that supports researchers and developers in efficiently implementing and validating novel strategies against baseline algorithms in Byzantine-resilient FL. Blades contains built-in implementations of representative attack and defense strategies and offers a user-friendly interface that seamlessly integrates new ideas. Using Blades, we re-evaluate representative attacks and defenses on wide-ranging experimental configurations (approximately 1,500 trials in total). Through our extensive experiments, we gained new insights into FL robustness and highlighted previously overlooked limitations due to the absence of thorough evaluations and comparisons of baselines under various attack settings.

==> attacks_and_defense.tex <==

% \begin{figure*}[!t]
% 	\centering
% 	\includegraphics[width=0.7\linewidth]{./figs/Blades_plots} '
% 	\caption{Overview of our classification of Byzantine attacks in FL. It indicates that adversaries at Levels 1 to 5 have different knowledge and control over the training, model, and strategy of different entities in the system. For instance, adversaries at Level 1 have control only on a single device, while they have control over the entire system at Level 5. %From Level 1 to 5, the 
%         }
% 	\label{fig_attacks}
% \end{figure*}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.98\linewidth]{./figs/attack_type.png}
    \vspace*{-.2cm}
	\caption{\small Overview of our classification of Byzantine attacks in FL. The diagram illustrates the relationship between different attack levels, where high-level attacks inherit the capabilities and knowledge of low-level attacks. The adversaries at Levels 1 to 5 have various degrees of knowledge and control capability over the dataset, model, and strategy of different entities in the system. 
 % For instance, adversaries at Level 1 control only a single device, while they control the entire system at Level 5. 
    }
\label{fig_attacks}
\end{figure}



\section{Systemization of Byzantine Attacks and Defenses}
\label{attack_defense_sec}
This section provides a systematic overview of Byzantine resilience in FL, encompassing key attack and defense techniques and other factors influencing robustness. \tv{motivate again that this is useful for the design of Blades}
% In this section, we introduce a five-level classification of Byzantine attacks, 
% categorized by the adversary's capabilities and knowledge. Then, we survey key 
% In this section, we perform a systematic study on Byzantine attacks and defenses in FL and discuss 
% In this study, we primarily focus on untargeted attacks in the context of Federated Learning (FL) systems. Section~\ref{subsec_fedavg} introduces a unified FL framework based on the famous \fedavg family algorithms. 
% Next, We  
% \ours contains high-quality implementations of popular attacks and defense strategies in FL.


% In contrast to distributed SGD, \fedavg-family algorithms perform several local steps of SGD before aggregation, which are designed to improve communication efficiency~\cite{reddi2020adaptive}.

% \input{pipeline}

\subsection{Classification of Byzantine Attacks in FL}
\label{attacks_sec}
On the basis of previous efforts for Byzantine attacks in FL, we classify these attacks into five levels in terms of the adversary's capabilities and knowledge. An overview of our classification system is illustrated in Fig.~\ref{fig_attacks}. Adversaries at higher levels have better knowledge and control over clients' training data and local models. Notably, adversaries at Level 5 even have complete knowledge of the FL system, including server-side defense strategies. 

% and  Examining each level of these attacks is essential for comprehending the security challenges encountered by FL systems. Through scrutinizing these assaults, we can discern their possible consequences and subsequently devise efficient defense mechanisms to ensure the security of FL systems.

% Studying each level of untargeted attacks is crucial to understanding the security threats faced by FL systems. By analyzing these attacks, we can identify their potential impact and develop effective defense strategies to safeguard the security of FL systems. In this work, we have directed our attention toward untargeted attacks in the federated learning (FL) setting. Untargeted attacks can be classified into five levels based on the adversary's capacity and knowledge.

% \myparatight{Data Poisoning Attacks (Level 1)} In this setting, an adversary has access to the training dataset of a single client but lacks knowledge of the model architecture, parameters, or outputs~\cite{rodriguez2023survey}\footnote{The term ``data poisoning" refers to the limited access to the data solely. Whilst advanced attacks (e.g., DLF~\cite{9833647}) utilize more information to modify training data accordingly, they are categorized as Level 2 in our classification.}. These attacks are relatively easy to launch since the attacker only requires minimal knowledge and access to the system.  For instance, an attacker could modify the labels of a dataset to introduce bias into the model or inject samples with subtle but harmful modifications~\cite{9650669,she3517821}. In turn, the lack of knowledge and access to the system may limit the effectiveness of Level 1 attacks. Moreover, it is possible to perform defense operations (e.g., gradient clipping) on the client's side during the local training phase, as the adversary cannot manipulate the training pipeline.

\myparatight{Naive Data Poisoning Attacks (Level 1)} At this level, the adversary possesses access to the training dataset of individual clients but
% \tv{before you write "an adversary," now "they." Be consistent (change "they" to "the adversary"}
lacks knowledge of the model's architecture, parameters, and outputs~\cite{rodriguez2023survey}\footnote{The term ``data poisoning'' specifically implies that the attacker's access is restricted to the dataset only, whereas sophisticated attacks to data such as DLF~\cite{9833647} are categorized as Level 2 due to their reliance on additional information for modifying the training data.}. These attacks are relatively straightforward to initiate, as they require minimal knowledge and access to the system. For example, an attacker could alter the labels of a dataset to introduce biases into the model or insert samples with subtle yet detrimental modifications~\cite{9650669,she3517821}. However, the limited knowledge and access to the system may restrict the effectiveness of attacks at this level. In addition,  except for server-side defenses, it is also feasible to implement defensive measures (e.g., gradient clipping) during the local training phase on the client's side, as the adversary cannot tamper with the training pipeline.


 \myparatight{Naive Model Poisoning Attacks (Level 2)} At this level, the adversary has complete control over a single participant, including access to the model parameters. They can manipulate the model updates transmitted to the server directly. Attacks at Level 2 and higher are referred to as ``Byzantine attacks''~\cite{li2023experimental} because the updates submitted by clients can be arbitrary. A straightforward Level 2 attack is to sample some random noise from a distribution (e.g., Gaussian distribution) and add it to the updates before communicating with the server~\cite{li2021byzantine}.

\myparatight{Collusion Attacks (Level 3)} At this level,  multiple malicious entities collude to compromise an FL system. These attacks are particularly challenging to defend against because the adversaries can share information with each other and coordinate their actions accordingly. In some cases, a single adversary may control a group of participants, e.g., by injecting fake clients to improve their effectiveness~\cite{Cao_2022_CVPR}. Adversaries at Level 3 and below face a trade-off between attack effectiveness and the risk of being detected by the server. The more effective an attack is, the higher the chance of it being detected by the server, which can lead to countermeasures such as client blocking~\cite{wan2022shielding, munoz2019byzantine}. On the other hand, if the adversary takes steps to reduce their detection risk, such as slowing down the attack or using more subtle methods, their attacks may not be effective. Therefore, attackers must carefully consider this trade-off when planning their strategies for collusion attacks in FL systems.

\myparatight{Limited Omniscient Attacks (Level 4)} In addition to the knowledge of malicious clients, the adversary at Level 4 possesses extra information about the benign clients, making them more dangerous than attackers at lower levels. This extra information may include model updates or local data distributions from benign clients, which allows the adversaries to craft more effective attacks. Due to access to peer information, attackers can conceal their identities by carefully crafting their updates and thus circumventing certain defense mechanisms. For instance, A Little is Enough (ALIE) attack~\cite{baruch2019little} assumes that the benign updates are expressed by a normal distribution. The attackers, therefore, can immediately take advantage of the high empirical variance between the updates of benign clients and upload a noise in a range without being detected.

\myparatight{Omniscient Attacks (Level 5)} The adversaries are assumed to have complete knowledge of the FL system, including server-side defense strategies. Level 5 attacks are often considered impractical to achieve in real-world settings due to the significant level of access and knowledge required, as noted in~\cite{9833647}. 
Nevertheless, it is essential to examine the probable impact of Level 5 attacks to identify vulnerabilities in defense strategies and to encourage the development of more effective security measures in FL systems.
% Despite this, we remark that studying the potential impact of Level 5 attacks is necessary because it helps to identify the vulnerabilities of a defense strategy and motivates the development of more effective security measures in FL systems. 
Level 5 attacks are generally known as ``adaptive attacks''~\cite{fang2020local}. In these attacks, adversaries develop malicious updates by solving an optimization problem aimed at maximizing the global model's damage in each local round, given their full knowledge of the local updates and defense strategies~\cite{shejwalkar2021manipulating,li2023experimental}.

% Typical Level 5 attacks are known as ``adaptive attacks''~\cite{fang2020local}, where the adversaries design malicious updates by solving an optimization problem that aims to maximize the damage to the global model in each local round, given the full knowledge of the local updates and defense strategies~\cite{shejwalkar2021manipulating,li2023experimental}.

It is worth noting that several taxonomies have already been proposed in the literature to categorize FL poisoning attacks~\cite{jere2020taxonomy,9833647}. In contrast, our new classification offers a few advantages for benchmarking attacks and defenses in FL. Firstly, it provides insights into the efficacy and limitations of attacks at different levels. Secondly, by categorizing attacks based on the adversary's skills and knowledge, our classification aids in conducting a thorough assessment of the robustness of defense mechanisms against different levels of threats. In turn, the proposed benchmark suite ensures an equitable and accurate evaluation of defenses. Additionally, the abstraction of the adversarial components in our simulator could benefit from the characteristics of our proposed attack classification, as shown in Section~\ref{sec_design}.

\input{tables/attack_table}

In Table~\ref{tb_atk}, we compare several representative attack strategies categorized by our classification system. For brevity and the sake of space limitation, we only choose six of them (shown in bold in Table~\ref{tb_atk}) to examine in this paper. Below we introduce these selected attacks in detail. 

\myparatight{LabelFlipping~\cite{pmlrv139karimireddy21a}} The adversary simply flips the label of each training sample~\cite{fang2020local}. Specifically, a label $l$ is flipped as $L-l-1$, where $L$ is the number of classes in the classification problem and $l=0,1,..., L-1$. 

\myparatight{SignFlipping~\cite{li2019rsa}} The adversary strives to maximize the loss via gradient ascent instead of gradient descent. Specifically, it flips the gradient's sign during the local updating step. 

\myparatight{Noise~\cite{li2021byzantine}} The adversary samples some random noise from a distribution (e.g., Gaussian distribution) and uploads it as local updates.

\myparatight{ALIE~\cite{baruch2019little}} The adversary takes advantage of the empirical variance among benign updates and uploads a noise within a range without being detected. For each coordinate $i \in [d]$, the attackers calculate mean ($\mu_i$) and std ($\delta_i$) over benign updates and set malicious updates to values in the range $(\mu_i - z^{max}\delta_i, \mu_i + z^{max}\delta_i)$, where $z^{max}$ ranges from 0 to 1, and is typically obtained from the Cumulative Standard Normal Function~\cite{baruch2019little}. The $i$-th malicious update is then obtained by $\Delta_{k,i}^t \leftarrow \mu_i - z^{max} \mu_i$.

\myparatight{IPM~\cite{xie2020fall}}
The adversary seeks the negative inner product between the true mean of the updates and the output of the aggregation rules so that the loss will at least not descend. Assuming that the attackers know the mean of benign updates, a specific way to perform an IPM attack is
	\begin{equation}
		\update_1^t = \dots = \update_M^t = - \frac{\epsilon}{K - M}\sum_{i = M+1}^K \update_i^t,
	\end{equation} where we assume that the first $M$ clients are malicious, $\epsilon$ is a positive coefficient controlling the magnitude of malicious updates.

\myparatight{MinMax~\cite{shejwalkar2021manipulating}} Similar to ALIE, the adversary strives to ensure that the malicious updates lie close to the clique of the benign updates. The difference is that MinMax re-scales $z^{max}$ such that the maximum distance from malicious updates to any benign updates is upper-bounded by the maximum distance between any two benign updates. 

\subsection{Defenses}
\label{sec_defense}
The defenses against Byzantine attacks primarily assume that only the server is trusted. Thus the defenses rely on server-side deployment.
% owing to the challenge of identifying malicious clients, as the server lacks supplementary information beyond local model updates. 
The literature has presented various directions toward mitigating the risks of Byzantine attacks in FL.

\input{tables/defense_table}

\subsubsection{Robust Aggregation}

The main branch of defense strategies strives to estimate the Byzantine-resilient global model update based on the local updates using robust aggregation rules~\cite{blanchard2017machine,yin2018byzantine,chen2017distributed,li2021byzantine,pmlrv139karimireddy21a,sattler2020byzantine}. Table~\ref{tb_defense} provides an overview of representative state-of-the-art aggregation rules. The column shows the corresponding characteristics shared by different rules. We only highlight three core characteristics upon which the majority of aggregation rules rely, i.e., Dimension-wise, Euclidean distance-wise, and Cosine distance-wise. Specifically, these rule aggregate involves comparing and aggregating updates based on either dimension-wise values, Euclidean distances, or directions. We categorize the rules into the following three groups:

\myparatight{Gradient Aggregation Rules (GAR)} Prior to the growing concern about Byzantine-resilient FL, the literature has already presented various directions toward making distributed machine learning robust against Byzantine or compromised nodes. The most typical techniques utilize robust aggregators to replace the average aggregation rule.

% , i.e., 
% \begin{equation}
%     \Delta^{t+1} \leftarrow \text{GAR}(\{g_k( \bm{w}_{k} ^ t)\}_{k\in [K]}),
% \end{equation} where $g_k( \bm{w}_{k} ^ t)$ is the estimated gradient.

When used within certain assumptions, classic GARs (e.g.,~\gm~\cite{chen2017distributed}, \krum~\cite{blanchard2017machine}, \tm~\cite{yin2018byzantine}, and \median~\cite{yin2018byzantine}) guarantee convergence even in an adversarial setting. However, the convergence guarantee applies only to distributed stochastic gradient descent (SGD), where the server aggregates local gradients reported by working machines and performs a gradient descent step. 

\myparatight{Extended Gradient Aggregation Rules (EGAR)} In contrast to traditional distributed SGD, \fedavg-family algorithms differentiate themselves by performing multiple local SGD steps at the client level, aiming to enhance communication efficiency~\cite{mcmahan2017communication}. Therefore, the aggregation rules are extended to aggregate gradient-like local updates (a.k.a. pseudo-gradients~\cite{reddi2020adaptive}).
% , i.e., 
% \begin{equation}
%     \Delta^{t+1} \leftarrow \text{EGAR}(\{\Delta_k^t\}_{k\in [K]}).
% \end{equation}


\myparatight{Weight Aggregation Rules (WAR)} Early studies proposed the adoption of robust aggregation techniques for model weight instead of gradients and updates~\cite{pillutla2022robust,munoz2019byzantine}. Although this category of techniques demonstrates a certain level of robustness in countering certain attacks, analyzing their convergence properties can be challenging~\cite{liconvergence}.

\fedavg-family algorithms often incorporate GARs~\cite{li2023experimental} initially proposed for distributed SGD, even though they lack convergence guarantee for multiple steps of local updates. Nevertheless, it is possible to integrate and conduct unified research and comparison between the two approaches to explore their combined potential, considering the utilization of local updates in \fedavg-family algorithms and the application of robust aggregation rules derived from distributed SGD. 

\subsubsection{Trust-based Strategies}
Trust-based strategies operate under the assumption that specific clients or datasets are considered trustworthy by the server~\cite{fang2020local,cao2021fltrust,9887909,sageflow}. The server, thereby, can re-weight and filter the local model updates according to various metrics, including empirical loss~\cite{fang2020local}, Cosine similarity\cite{cao2021fltrust}, and entropy~\cite{sageflow}.

Compared to robust aggregation rules, trust-based strategies exhibit the potential to address the case where the majority of clients are malicious. Nonetheless, the availability of trustworthy datasets or clients for the server is not always guaranteed, primarily due to concerns regarding user data privacy.

\subsubsection{Variance-reduced Algorithms} 
Variance reduction techniques have been recognized for their significance in improving the robustness of FL against Byzantine attacks~\cite{gorbunov2023variance}. Previous research in GAR has highlighted that the bounded variance of benign gradients plays a critical role in the Byzantine tolerance of malicious nodes~\cite{chen2017distributed,yin2018byzantine}, inspiring the development of variance-reduced algorithms~\cite{gorbunov2023variance,9153949}. 

The core idea of variance-reduced algorithms is to reduce the stochastic noise of gradient estimators used by benign clients, thereby making it easier to filter out Byzantine gradients. Byrd-SAGA, for instance, combines the celebrated SAGA method~\cite{defazio2014saga} with the \gm aggregation rule. It is noteworthy that variance-reduced algorithms act as supportive mechanisms and require concurrent utilization with robust aggregation rules to attain robustness. They are currently used exclusively in distributed SGD settings and are incompatible with multiple local steps on the client side. Such a characteristic imposes limitations on the optimization's communication efficiency.

\subsubsection{Additional Defense Techniques} In addition to the aforementioned categories, a range of supplementary defense techniques offer further enhancements to the security and robustness of FL systems. While these techniques do not fit explicitly into the previously defined categories, they are still significant in the context of FL defense.

% These techniques, although not fitting explicitly into the previously defined categories, are nonetheless significant in the context of federated learning defense. 

\label{additional_defense}
\myparatight{Momentum} In the context of Byzantine-resilient FL, momentum was initially introduced to reduce the variance of local updates~\cite{pmlrv139karimireddy21a}. Recent studies have shown that distributed momentum could improve existing defenses against state-of-the-art attacks~\cite{mhamdi2021distributed,pmlrv162farhadkhani22a,gu2023dp}. Specifically, each client maintains the momentum by accumulating historical gradients and uploading it for aggregation. When distributed momentum is employed, the local model optimization process considers the historical momentum accumulated from the clients themselves. As a result, the impact of Byzantine updates is reduced because the aggregated momentum tends to smooth out the influence of malicious updates.

\myparatight{Clipping} Some aggregation rules enhance robustness by performing clipping (Table~\ref{tb_defense}) on all the updates in advance:
\begin{equation}
  \Delta_{k}^t \leftarrow \Delta_{k}^t\min(1, \frac{\tau}{\lVert \Delta_k^t \rVert}),
\end{equation} where $\tau$ is a hyper-parameter of the clipping value, which is determined by the server. The underlying intuition is to mitigate the impact of adversarial updates that could lead to substantial model deviations. In addition, it is worth noting that the risk of gradient explosion, as revealed by our experiments, could also be mitigated by clipping gradients~\cite{goodfellow2016deep}. See Section~\ref{sec_gradient_explosion} for more details.

% \myparatight{Bucketing}


\subsection{Other Factors Influencing Robustness}

Apart from attack and defense strategies, there are other factors that influence the robustness of the optimization process, such as differential privacy and data heterogeneity. 



\myparatight{Noise-adding for Differential Privacy (DP)} One of the most common approaches to building a DP-based mechanism is to use Gaussian noise injection~\cite{andrew2021differentially,dwork2008differential}. According to prior art~\cite{dwork2008differential}, the noisy updates

\begin{equation}
	\widetilde{ \Delta}_k^t \leftarrow  \Delta_k^t + \mathbf{y}_k^t,
\end{equation}
with $\mathbf{y}_k^t \sim N(0, I_d \times s^2)$ where $s = \frac{2G_{max} \sqrt{2\log{(1.25/\delta)}}}{b\epsilon}$, sent by client $k$ is $(\epsilon, \delta)$--differential private. Given a privacy budget $(\epsilon, \delta)$, the privacy guarantees of the overall learning procedure can be determined by leveraging the composition property of DP. The robustness guarantee of robust aggregation rules depends on the low variance of client stochastic gradients. However, the Gaussian DP mechanism adds random noise to the gradients, which can increase the variance especially when the DP budget is low (e.g., when $\epsilon$ and $\delta$ approach 0), making it more difficult to satisfy the robustness conditions~\cite{yin2018byzantine}.

\myparatight{Data Heterogeneity}  As noted in prior studies~\cite{fang2020local,karimireddy2022byzantinerobust,li2023experimental}, the presence of data heterogeneity imposes additional challenges on the exclusion of the influence of malicious updates in FL. Higher levels of data heterogeneity result in increased diversity in the local updates, making it more challenging to identify and exclude the effects of malicious updates.

% Specifically, heightened levels of heterogeneity amplify the diversity of local updates, thereby complicating the defenses of identifying and excluding the effects of malicious updates.  


% \myparatight{Local Steps} 

% \input{pipeline}

==> pipeline.tex <==
\subsection{A Generic Pipeline}
% \subsection{Unifying Byzantine Fault-Tolerant Distributed SGD with FL}
\label{subsec_fedavg}


Additionally, it is possible to extend \fedavg-family algorithms by incorporating a broader range of operations at both the server and client levels. These additional operations can encompass various aspects of the federated learning process, such as Noise-adding for differential privacy (DP)~\cite{dwork2008differential}, trusted data validation~\cite{cao2021fltrust}, and adaptive learning strategies~\cite{reddi2020adaptive,munoz2019byzantine}. This extension goes beyond the traditional tasks of gradient updating and aggregation, which has implications for the robustness of FL against attacks.

To address these diverse aspects, we propose a unified framework at a high level for studying the challenges associated with Byzantine attacks and defenses in federated learning, encompassing elements such as robust aggregation, local updates, communication efficiency, privacy preservation, and adaptive strategies. This framework would serve as a foundation for researching the challenges related to Byzantine attacks and defenses in FL and inspire us to design and develop a benchmark suite specifically tailored for studying this problem.

==> pipeline_bk.tex <==
\subsection{A Generic Pipeline}
% \subsection{Unifying Byzantine Fault-Tolerant Distributed SGD with FL}
\label{subsec_fedavg}
Prior to the growing concern about Byzantine-resilient FL, the literature has already presented various directions toward making distributed machine learning robust against Byzantine or compromised nodes. The major branch of techniques utilizes robust aggregators to replace the average aggregation rule. When used within its operating assumptions, classic schemes, including~\gm~\cite{chen2017distributed}, \krum~\cite{blanchard2017machine}, \tm~\cite{yin2018byzantine}, and \median~\cite{yin2018byzantine}, guarantee convergence even in an adversarial setting. Notably, the convergence guarantee only applies to distributed SGD, where the parameter aggregates the local gradients reported by the working machines and performs a gradient descent step.


In contrast to traditional distributed SGD, \fedavg-family algorithms differentiate themselves by performing multiple local SGD steps at the client level, aiming to enhance communication efficiency~\cite{mcmahan2017communication}. However, these \fedavg-family algorithms sometimes incorporate the aforementioned robust aggregation rules~\cite{li2023experimental}, which were initially proposed for distributed SGD. Hence, there is a need to integrate and conduct unified research and comparison between the two approaches to explore their combined potential, considering the utilization of local updates in \fedavg-family algorithms and the application of robust aggregation rules derived from distributed SGD.

Additionally, it is possible to extend \fedavg-family algorithms by incorporating a broader range of operations at both the server and client levels. These additional operations can encompass various aspects of the federated learning process, such as Noise-adding for differential privacy (DP)~\cite{dwork2008differential}, trusted data validation~\cite{cao2021fltrust}, and adaptive learning strategies~\cite{reddi2020adaptive,munoz2019byzantine}. This extension goes beyond the traditional tasks of gradient updating and aggregation, which in turn, has implications for the robustness of FL against attacks.

To address these diverse aspects, we propose a unified framework at a high level for studying the challenges associated with Byzantine attacks and defenses in federated learning, encompassing elements such as robust aggregation, local updates, communication efficiency, privacy preservation, and adaptive strategies. This framework would serve as a foundation for researching the challenges related to Byzantine attacks and defenses in FL and inspire us to design and develop a benchmark suite specifically tailored for studying this problem.

==> tables/agr_bk.tex <==
\newcommand \alignline{ \cline{2-12}}
\newcommand \thickvline{ \color{black}\vline width 1pt}
\newcommand{\rotbox}[1]{\rotatebox[origin=c]{75}{#1}}
\begin{table*}[]
\setlength\extrarowheight{3pt}
\begin{adjustbox}{width=0.9\textwidth,center}

\begin{tabular}{!{\color{black}\vline width 1pt}c!{\thickvline}c!{\thickvline}c|c|c|c|c|c|c|c!{\color{black}\vline width 1pt}>
{\columncolor[gray]{0.9}}
c!{\color{black}\vline width 1pt}c!{\thickvline}}

\Xhline{3\arrayrulewidth}
 &  & \multicolumn{8}{c!{\color{black}\vline width 1pt}}{Machanisms}  &  & \\
\hline
 Aggregation Type& Reference & \rotbox{Dimension-wise} & \rotbox{\makecell{Euclidean  Distance}} & \rotbox{Cosine Distance} & \rotbox{Eigenvector} & \rotbox{Clipping} & \rotbox{Stateful} &  \rotbox{Sign-based} &  \rotbox{\makecell{Median-based}}  & \rotbox{\makecell{Time \\ Complexity}}& Description \\
\Xhline{3\arrayrulewidth}
 \multirow{5}{*}{\makecell{Robust Gradient \\ Aggregation}}   &      Krum~\cite{blanchard2017machine}, Multi-Krum~\cite{blanchard2017machine}     &      & \checkmark  &  &  &  &  &  &  & $n\log n$ &\\
\alignline
& GeoMed~\cite{chen2017distributed}   & & \checkmark & &  &  & & &  \checkmark && \\
\alignline
 &  Median~\cite{yin2018byzantine} & \checkmark  &&& & & & & \checkmark  & & \\
\alignline
& TrimmedMean~\cite{yin2018byzantine}     & \checkmark  & & & &  & & &  & & \\ 
\alignline
     &  SignSGD-MV~\cite{bernstein2018signsgd}      & \checkmark                    &          &          &                 &          &                 & \checkmark      &  & & \multirow{1}{*}{Communication efficient}  \\
\hline  
 \multirow{7}{*}{\makecell{Extended Robust  \\ Aggregation}} &    Signguard~\cite{xu2022byzantine} &   &  & &  & \checkmark &  & \checkmark      &   \checkmark  &  &\\
\alignline
&   RAGE~\cite{data2021byzantine} &   &  & &    \checkmark &  &  &  & & & \\
\alignline
 &    DnC~\cite{shejwalkar2021manipulating}  &  &  & &  \checkmark & &  &  & & & \\
\alignline
&   AutoGM~\cite{li2021byzantine}  &  & \checkmark  & & & & & &  \checkmark & & \\
\alignline
&   MAB-RFL~\cite{wan2022shielding}   &   &  &  \checkmark   &  &  &\checkmark    & & & & \\
\alignline
 &  Clustering~\cite{sattler2020byzantine} &   & &   \checkmark  & && & & & & \\
\alignline
  &   ClippedClustering~\cite{li2023experimental} & & & \checkmark  & & \checkmark   & \checkmark &&  \checkmark   &  & \\
\hline 
\multirow{2}{*}{\makecell{Weight Aggregation}} & RFA~\cite{pillutla2022robust} & & \checkmark &  &  & &  & & \checkmark  &   & \\
\alignline
&    AFA~\cite{munoz2019byzantine}   & & &  \checkmark   & & & \checkmark &&& & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\end{adjustbox}
\caption{A summary of robust aggregation strategies.}
\label{tb_agr}
\end{table*}


==> tables/attack_table.tex <==
\begin{table}[!t]
% \newcommand \alignline{ \cline{1-7}}
\newcommand \alignline{ }
\newcommand \thickvline{ \color{black}\vline width 1pt}
\newcommand{\rotbox}[1]{\rotatebox[origin=c]{0}{#1}}
\caption{Example attack strategies grouped according to our classification system. 
}
% \vspace*{-.3cm}
\setlength\extrarowheight{3pt}
\setlength{\arrayrulewidth}{0.3mm}
\begin{adjustbox}{width=0.85\linewidth,center}

% \begin{tabular}{c|c|c|c|c|c|cc}
\begin{tabular}{c|ccccccc}

\hline
 \multirow{2}{*}{\textbf{Attack}} & \multicolumn{5}{c}{\textbf{Level of Knowledge and capability}} \\
\cline{2-7}
  & Level 1 & Level 2 & Level 3 & Level 4 & Level 5  \\
\hline
\hline
  \textbf{LabelFlipping}~\cite{pmlrv139karimireddy21a}  & \Checkmark  &  &&&\\
\alignline
  \textbf{SignFlipping}~\cite{li2019rsa}  && \Checkmark &&&\\
\alignline  
  \textbf{Noise}~\cite{li2021byzantine}  && \Checkmark &&&\\
\alignline  
MPAF~\cite{Cao_2022_CVPR} & \Checkmark & & \Checkmark &  & \\
\alignline
   \textbf{ALIE}~\cite{baruch2019little}       &  & \Checkmark & \Checkmark & \Checkmark &  \\
\alignline
     DPA~\cite{9833647}       & \Checkmark & \Checkmark & \Checkmark & \Checkmark &  \\
\alignline
    \textbf{IPM}~\cite{xie2020fall} & & & \Checkmark & \Checkmark &   \\
\alignline
    \textbf{MinMax}~\cite{shejwalkar2021manipulating} &  & \Checkmark & \Checkmark & \Checkmark & \\
\alignline
    Fang Attack~\cite{karimireddy2022byzantinerobust} &  & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
\alignline
    AGR-tailored Attack~\cite{shejwalkar2021manipulating} &  & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
\hline

\end{tabular}
\end{adjustbox}
\label{tb_atk}
\end{table}


==> tables/attack_table_bk.tex <==
\begin{table*}[ht]
\newcommand \alignline{ \cline{2-7}}
\newcommand \thickvline{ \color{black}\vline width 1pt}
\newcommand{\rotbox}[1]{\rotatebox[origin=c]{0}{#1}}
\caption{A summary of attack strategies.}
\setlength\extrarowheight{3pt}
\begin{adjustbox}{width=0.75\textwidth,center}

\begin{tabular}{!{\color{black}\vline width 1pt}c|c!{\thickvline}c!{\thickvline}c|c|c|c!{\color{black}\vline width 1pt}>
{\columncolor[gray]{0.9}}
c!{\color{black}\vline width 1pt}l!{\thickvline}}

\Xhline{3\arrayrulewidth}
Type & Reference & \multicolumn{5}{c!{\color{black}\vline width 1pt}}{Knowledge level} & Description\\
\hline
\hline
   % &  & \rotbox{Global model} & \rotbox{\makecell{Local data}} & \rotbox{\makecell{Adversary's \\ knowledge}} & \rotbox{\makecell{All client's \\ knowledge}} & \rotbox{\makecell{Defense \\ strategy}} &  \\
      &  & L1 & L2 & L3 & L4 & L5 &  \\

\hline
\hline

\multicolumn{1}{|c|}{\multirow{2}{*}{Data Poisoning}}
&   Labelflipping~\cite{pmlrv139karimireddy21a}  & \checkmark &  &&&&\\
\alignline
\multicolumn{1}{|c|}{}&    DPA~\cite{9833647}       & \checkmark & \checkmark & \checkmark & \checkmark & & \\
\hline
\hline

\multicolumn{1}{|c|}{\multirow{6}{*}{Model Poisoning}}
&   Signflipping~\cite{li2019rsa}  && \checkmark &&&&\\
\alignline
\multicolumn{1}{|c|}{}&     
MPAF~\cite{Cao_2022_CVPR} & \checkmark & & \checkmark &  & &\\
\alignline
\multicolumn{1}{|c|}{}&    ALIE~\cite{baruch2019little}       &  & \checkmark & \checkmark & \checkmark & & \\
\alignline
\multicolumn{1}{|c|}{}&     IPM~\cite{xie2020fall} & & & \checkmark & \checkmark &  & \\
\alignline
\multicolumn{1}{|c|}{}&     Fang Attack~\cite{karimireddy2022byzantinerobust} &  & \checkmark & \checkmark & \checkmark & \checkmark &\\
\alignline
\multicolumn{1}{|c|}{}&     AGR-tailored Attack~\cite{shejwalkar2021manipulating} &  & \checkmark & \checkmark & \checkmark & \checkmark &\\
\Xhline{3\arrayrulewidth}

\end{tabular}
\end{adjustbox}
\label{tb_agr}
\end{table*}


==> tables/attacks_and_defense.tex <==

% \begin{figure*}[!t]
% 	\centering
% 	\includegraphics[width=0.7\linewidth]{./figs/Blades_plots}
% 	\caption{Overview of our classification of Byzantine attacks in FL. It indicates that adversaries at Levels 1 to 5 have different knowledge and control over the training, model, and strategy of different entities in the system. For instance, adversaries at Level 1 have control only on a single device, while they have control over the entire system at Level 5. %From Level 1 to 5, the 
%         }
% 	\label{fig_attacks}
% \end{figure*}

\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{./figs/attack_type}
	\caption{\small Overview of our classification of Byzantine attacks in FL. The diagram illustrates the relationship between different attack levels, where high-level attacks inherit the capabilities and knowledge of low-level attacks (indicated by red arrows). The adversaries at Levels 1 to 5 have various degrees of knowledge and control over the dataset, model, and strategy of different entities in the system. For instance, adversaries at Level 1 have control only over a single device, while they have control over the entire system at Level 5. 
    }
\label{fig_attacks}
\end{figure}



\section{Byzantine Attacks and Defenses}
\label{attack_defense_sec}
This section provides a systematic overview of Byzantine resilience in FL, encompassing key attack and defense techniques and other factors that influence robustness.
% In this section, we start by introducing a five-level classification of Byzantine attacks, 
% categorized by the adversary's capabilities and knowledge. Then, we survey key 
% In this section, we perform a systematic study on Byzantine attacks and defenses in FL, and discuss 
% In this study, we primarily focus on untargeted attacks in the context of Federated Learning (FL) systems. Section~\ref{subsec_fedavg} introduces a unified FL framework based on the famous \fedavg family algorithms. 
% Next, We  
% \ours contains high-quality implementations of popular attacks and defense strategies in FL.


% In contrast to distributed SGD, \fedavg-family algorithms perform several local steps of SGD before aggregation, which are designed to improve communication efficiency~\cite{reddi2020adaptive}.

% \input{pipeline}

\subsection{Classification of Byzantine Attacks in FL}
\label{attacks_sec}
On the basis of previous efforts for Byzantine attacks in FL, we classify these attacks into five levels in terms of the adversary's capabilities and knowledge. An overview of our classification system is illustrated in Fig.~\ref{fig_attacks}. Adversaries at higher levels have better knowledge and control over clients' training data and local models. Notably, adversaries at Level 5 even have complete knowledge of the FL system, including server-side defense strategies. 

% and  Examining each level of these attacks is essential for comprehending the security challenges encountered by FL systems. Through scrutinizing these assaults, we can discern their possible consequences and subsequently devise efficient defense mechanisms to ensure the security of FL systems.

% Studying each level of untargeted attacks is crucial to understanding the security threats faced by FL systems. By analyzing these attacks, we can identify their potential impact and develop effective defense strategies to safeguard the security of FL systems. In this work, we have directed our attention toward untargeted attacks in the federated learning (FL) setting. Untargeted attacks can be classified into five levels based on the adversary's capacity and knowledge.

% \myparatight{Data Poisoning Attacks (Level 1)} In this setting, an adversary has access to the training dataset of a single client but lacks knowledge of the model architecture, parameters, or outputs~\cite{rodriguez2023survey}\footnote{The term ``data poisoning" refers to the limited access to the data solely. Whilst advanced attacks (e.g., DLF~\cite{9833647}) utilize more information to modify training data accordingly, they are categorized as Level 2 in our classification.}. These attacks are relatively easy to launch since the attacker only requires minimal knowledge and access to the system.  For instance, an attacker could modify the labels of a dataset to introduce bias into the model or inject samples with subtle but harmful modifications~\cite{9650669,she3517821}. In turn, the lack of knowledge and access to the system may limit the effectiveness of Level 1 attacks. Moreover, it is possible to perform defense operations (e.g., gradient clipping) on the client's side during the local training phase, as the adversary cannot manipulate the training pipeline.

\myparatight{Naive Data Poisoning Attacks (Level 1)} At this level, the adversary possesses access to the training dataset of individual clients but
% \tv{before you write "an adversary," now "they." Be consistent (change "they" to "the adversary"}
lacks knowledge of the model's architecture, parameters, and outputs~\cite{rodriguez2023survey}\footnote{The term ``data poisoning'' specifically implies that the attacker's access is restricted to the dataset only, whereas sophisticated attacks to data such as DLF~\cite{9833647} are categorized as Level 2 due to their reliance on  additional information for modifying the training data.}. These attacks are relatively straightforward to initiate, as they require minimal knowledge and access to the system. For example, an attacker could alter the labels of a dataset to introduce biases into the model or insert samples with subtle yet detrimental modifications~\cite{9650669,she3517821}. However, the limited knowledge and access to the system may restrict the effectiveness of attacks at this level. In addition,  except for server-side defenses, it is also feasible to implement defensive measures (e.g., gradient clipping) during the local training phase on the client's side, as the adversary cannot tamper with the training pipeline.


 \myparatight{Naive Model Poisoning Attacks (Level 2)} At this level, the adversary has complete control over a single participant, including access to the model parameters. They can manipulate the model updates transmitted to the server directly. Attacks at Level 2 and higher are referred to as ``Byzantine attacks''~\cite{li2023experimental} because the updates submitted by clients can be arbitrary. A straightforward Level 2 attack is to sample some random noise from a distribution (e.g., Gaussian distribution) and add it to the updates before communicating with the server~\cite{li2021byzantine}.

\myparatight{Collusion Attacks (Level 3)} At this level,  multiple malicious entities collude to compromise an FL system. These attacks are particularly challenging to defend against because the adversaries can share information with each other and coordinate their actions accordingly. In some cases, a single adversary may control a group of participants, e.g., by injecting fake clients to improve their effectiveness~\cite{Cao_2022_CVPR}. Adversaries at Level 3 and below face a trade-off between attack effectiveness and the risk of being detected by the server. The more effective an attack is, the higher the chance of it being detected by the server, which can lead to countermeasures such as client blocking~\cite{wan2022shielding, munoz2019byzantine}. On the other hand, if the adversary takes steps to reduce their detection risk, such as slowing down the attack or using more subtle methods, their attacks may not be  effective. Therefore, attackers must carefully consider this trade-off when planning their strategies for collusion attacks in FL systems.

\myparatight{Limited Omniscient Attacks (Level 4)} In addition to the knowledge of malicious clients, the adversary at Level 4 possesses extra information about the benign clients, making them more dangerous than attackers at lower levels. This extra information may include model updates or local data distributions from benign clients, which allows the adversaries to craft more effective attacks. Due to access to peer information, attackers can conceal their identities by carefully crafting their updates and thus circumventing certain defense mechanisms. For instance, A Little is Enough (ALIE) attack~\cite{baruch2019little} assumes that the benign updates are expressed by a normal distribution. The attackers, therefore, can immediately take advantage of the high empirical variance between the updates of benign clients and upload a noise in a range without being detected.

\myparatight{Omniscient Attacks (Level 5)} The adversaries are assumed to have complete knowledge of the FL system, including server-side defense strategies. Level 5 attacks are often considered impractical to achieve in real-world settings due to the significant level of access and knowledge required, as noted in~\cite{9833647}. 
Nevertheless, it is essential to examine the probable impact of Level 5 attacks to identify vulnerabilities in defense strategies and to encourage the development of more effective security measures in FL systems.
% Despite this, we remark that studying the potential impact of Level 5 attacks is necessary because it helps to identify the vulnerabilities of a defense strategy and motivates the development of more effective security measures in FL systems. 
Level 5 attacks are generally known as ``adaptive attacks''~\cite{fang2020local}. In these attacks, adversaries develop malicious updates by solving an optimization problem aimed at maximizing the global model's damage in each local round, given their full knowledge of the local updates and defense strategies~\cite{shejwalkar2021manipulating,li2023experimental}.

% Typical Level 5 attacks are known as ``adaptive attacks''~\cite{fang2020local}, where the adversaries design malicious updates by solving an optimization problem that aims to maximize the damage to the global model in each local round, given the full knowledge of the local updates and defense strategies~\cite{shejwalkar2021manipulating,li2023experimental}.

It is worth noting that several taxonomies have already been proposed in the literature to categorize FL poisoning attacks~\cite{jere2020taxonomy,9833647}. In contrast, our new classification offers a few advantages for benchmarking attacks and defenses in FL. Firstly, it provides insights into the efficacy and limitations of attacks at different levels. Secondly, by categorizing attacks based on the adversary's skills and knowledge, our classification aids in conducting a thorough assessment of the robustness of defense mechanisms against different levels of threats. In turn, the proposed benchmark suite ensures an equitable and accurate evaluation of defenses. Additionally, the abstraction of the adversarial components in our simulator could benefit from the characteristics of our proposed attack classification, as shown in Section~\ref{sec_design}.

\input{tables/attack_table}

In Table~\ref{tb_atk}, we compare several representative attack strategies categorized by our classification system. For brevity and the sake of space limitation, we only choose six of them (shown in bold in Table~\ref{tb_atk}) to examine in this paper. Below we introduce these selected attacks in detail. 

\input{tables/defense_table}

\myparatight{LabelFlipping~\cite{pmlrv139karimireddy21a}} The adversary simply flips the label of each training sample~\cite{fang2020local}. Specifically, a label $l$ is flipped as $L-l-1$, where $L$ is the number of classes in the classification problem and $l=0,1,..., L-1$.

\myparatight{SignFlipping~\cite{li2019rsa}} The adversary strives to maximize the loss via gradient ascent instead of gradient descent. Specifically, it flips the gradient's sign during the local updating step. 

\myparatight{Noise~\cite{li2021byzantine}} The adversary samples some random noise from a distribution (e.g., Gaussian distribution) and uploads it as local updates.

\myparatight{ALIE~\cite{baruch2019little}} The adversary takes advantage of the empirical variance among benign updates and uploads a noise within a range without being detected. For each coordinate $i \in [d]$, the attackers calculate mean ($\mu_i$) and std ($\delta_i$) over benign updates and set malicious updates to values in the range $(\mu_i - z^{max}\delta_i, \mu_i + z^{max}\delta_i)$, where $z^{max}$ ranges from 0 to 1, and is typically obtained from the Cumulative Standard Normal Function~\cite{baruch2019little}. The $i$-th malicious update is then obtained by $\Delta_{k,i}^t \leftarrow \mu_i - z^{max} \mu_i$.

\myparatight{IPM~\cite{xie2020fall}}
The adversary seeks the negative inner product between the true mean of the updates and the output of the aggregation rules so that the loss will at least not descend. Assuming that the attackers know the mean of benign updates, a specific way to perform an IPM attack is
	\begin{equation}
		\update_1^t = \dots = \update_M^t = - \frac{\epsilon}{K - M}\sum_{i = M+1}^K \update_i^t,
	\end{equation} where we assume that the first $M$ clients are malicious, $\epsilon$ is a positive coefficient controlling the magnitude of malicious updates.

\myparatight{MinMax~\cite{shejwalkar2021manipulating}} Similar to ALIE, the adversary strives to ensure that the malicious updates lie close to the clique of the benign updates. The difference is that MinMax re-scales $z^{max}$ such that the maximum distance from malicious updates to any benign updates is upper-bounded by the maximum distance between any two benign updates. 

\subsection{Defenses}
\label{sec_defense}
The defenses against Byzantine attacks primarily assume that only the server is trusted. Thus the defenses rely on server-side deployment.
% owing to the challenge of identifying malicious clients, as the server lacks supplementary information beyond local model updates. 
The literature has presented various directions toward mitigating the risks posed by Byzantine attacks in FL.

\subsubsection{Robust Aggregation}

The main branch of defense strategies strives to estimate the Byzantine-resilient global model update based on the local updates using robust aggregation rules~\cite{blanchard2017machine,yin2018byzantine,chen2017distributed,li2021byzantine,karimireddy2021learning,sattler2020byzantine}. Table~\ref{tb_defense} provides an overview of representative state-of-the-art aggregation rules. The column shows the corresponding characteristics shared by different rules. We only highlight three core characteristics upon which the majority of aggregation rules rely, i.e., Dimension-wise, Euclidean distance-wise, and Cosine distance-wise. Specifically, these rule aggregate involves comparing and aggregating updates based on either dimension-wise values, Euclidean distances, or directions.

In the aggregation type dimension, we categorize the rules into the following three groups:

\myparatight{Gradient
Aggregation Rules (GAR)} Prior to the growing concern about Byzantine-resilient FL, the literature has already presented various directions toward making distributed machine learning robust against Byzantine or compromised nodes. The most typical techniques utilize robust aggregators to replace the average aggregation rule.

% , i.e., 
% \begin{equation}
%     \Delta^{t+1} \leftarrow \text{GAR}(\{g_k( \bm{w}_{k} ^ t)\}_{k\in [K]}),
% \end{equation} where $g_k( \bm{w}_{k} ^ t)$ is the estimated gradient.

% The major branch of

When used within certain assumptions, classic GARs (e.g.,~\gm~\cite{chen2017distributed}, \krum~\cite{blanchard2017machine}, \tm~\cite{yin2018byzantine}, and \median~\cite{yin2018byzantine}) guarantee convergence even in an adversarial setting. However, the convergence guarantee applies only to distributed stochastic gradient descent (SGD), where the server aggregates local gradients reported by working machines and performs a gradient descent step. 

\myparatight{Extended Gradient Aggregation Rules (EGAR)} In contrast to traditional distributed SGD, \fedavg-family algorithms differentiate themselves by performing multiple local SGD steps at the client level, aiming to enhance communication efficiency~\cite{mcmahan2017communication}. Therefore, the aggregation rules are extended to aggregate gradient-like local updates (a.k.a. pseudo-gradients~\cite{reddi2020adaptive}).
% , i.e., 
% \begin{equation}
%     \Delta^{t+1} \leftarrow \text{EGAR}(\{\Delta_k^t\}_{k\in [K]}).
% \end{equation}


\myparatight{Weight Aggregation Rules (WAR)} Early studies proposed the adoption of robust aggregation techniques for model weight instead of gradients and updates~\cite{pillutla2022robust,munoz2019byzantine}. Although this category of techniques demonstrates a certain level of robustness in countering certain attacks, analyzing their convergence properties can be challenging~\cite{liconvergence}.

\fedavg-family algorithms often incorporate GARs~\cite{li2023experimental} initially proposed for distributed SGD, even though they lack convergence guarantee for multiple steps of local updates. Nevertheless, it is possible to integrate and conduct unified research and comparison between the two approaches to explore their combined potential, considering the utilization of local updates in \fedavg-family algorithms and the application of robust aggregation rules derived from distributed SGD. 

\subsubsection{Trust-based Strategies}
Trust-based strategies operate under the assumption that specific clients or datasets are considered trustworthy by the server~\cite{fang2020local,cao2021fltrust,9887909,sageflow}. The server, thereby, can re-weight and filter the local model updates according to various metrics, including empirical loss~\cite{fang2020local}, Cosine similarity\cite{cao2021fltrust}, and entropy~\cite{sageflow}.

Compared to robust aggregation rules, trust-based strategies exhibit the potential to address the case where the majority of clients are malicious. Nonetheless, the availability of trustworthy datasets or clients for the server is not always guaranteed, primarily due to concerns regarding user data privacy.

\subsubsection{Variance-reduced Algorithms} 
Variance reduction techniques have been recognized for their significance in improving the robustness of FL against Byzantine attacks~\cite{gorbunov2023variance}. Previous research in GAR has highlighted that the bounded variance of benign gradients plays a critical role in the Byzantine tolerance of malicious nodes~\cite{chen2017distributed,yin2018byzantine}, inspiring the development of variance-reduced algorithms~\cite{gorbunov2023variance,9153949}. 

The core idea of variance-reduced algorithms is to reduce the stochastic noise of gradient estimators used by benign clients, thereby making it easier to filter out Byzantine gradients. Byrd-SAGA, for instance, combines the celebrated SAGA method~\cite{defazio2014saga} with the \gm aggregation rule. It is noteworthy that variance-reduced algorithms act as supportive mechanisms and require concurrent utilization with robust aggregation rules to attain robustness. They are currently used exclusively in distributed SGD settings and are incompatible with multiple local steps on the client side. Such a characteristic imposes limitations on the optimization's communication efficiency.

\subsubsection{Additional Defense Techniques} In addition to the aforementioned categories, a range of supplementary defense techniques offer further enhancements to the security and robustness of FL systems. While these techniques do not fit explicitly into the previously defined categories, they are still significant in the context of FL defense.

% These techniques, although not fitting explicitly into the previously defined categories, are nonetheless significant in the context of federated learning defense. 

\label{additional_defense}
\myparatight{Momentum} In the context of Byzantine-resilient FL, momentum was initially introduced to reduce the variance of local updates~\cite{pmlrv139karimireddy21a}. Recent studies have shown that distributed momentum could improve existing defenses against state-of-the-art attacks~\cite{mhamdi2021distributed,pmlrv162farhadkhani22a,gu2023dp}. Specifically, each client maintains the momentum by accumulating historical gradients and uploading it for aggregation. When distributed momentum is employed, the local model optimization process considers the historical momentum accumulated from the clients themselves. As a result, the impact of Byzantine updates is reduced because the aggregated momentum tends to smooth out the influence of malicious updates.

\myparatight{Clipping} Some aggregation rules enhance robustness by performing clipping (Table~\ref{tb_defense}) on all the updates in advance:
\begin{equation}
  \Delta_{k}^t \leftarrow \Delta_{k}^t\min(1, \frac{\tau}{\lVert \Delta_k^t \rVert}),
\end{equation} where $\tau$ is a hyper-parameter of the clipping value, which is determined by the server. The underlying intuition is to mitigate the impact of adversarial updates that could lead to substantial model deviations. In addition, it is worth noting that the risk of gradient explosion, as revealed by our experiments, could also be mitigated by clipping gradients~\cite{goodfellow2016deep}. See Section~\ref{sec_gradient_explosion} for more details.

% \myparatight{Bucketing}


\subsection{Other Factors Influencing Robustness}

Apart from attack and defense strategies, there are other factors that influence the robustness of the optimization process, such as differential privacy and data heterogeneity. 



\myparatight{Noise-adding for Differential Privacy (DP)} One of the most common approaches to building a DP-based mechanism is to use Gaussian noise injection~\cite{andrew2021differentially,dwork2008differential}. According to prior art~\cite{dwork2008differential}, the noisy updates

\begin{equation}
	\widetilde{ \Delta}_k^t \leftarrow  \Delta_k^t + \mathbf{y}_k^t,
\end{equation}
with $\mathbf{y}_k^t \sim N(0, I_d \times s^2)$ where $s = \frac{2G_{max} \sqrt{2\log{(1.25/\delta)}}}{b\epsilon}$, sent by client $k$ is $(\epsilon, \delta)$--differential private. Given a privacy budget $(\epsilon, \delta)$, the privacy guarantees of the overall learning procedure can be determined by leveraging the composition property of DP. The robustness guarantee of robust aggregation rules depends on the low variance of client stochastic gradients. However, the Gaussian DP mechanism adds random noise to the gradients, which can increase the variance especially when the DP budget is low (e.g., when $\epsilon$ and $\delta$ approach 0), making it more difficult to satisfy the robustness conditions~\cite{yin2018byzantine}.

\myparatight{Data Heterogeneity}  As noted in prior studies~\cite{fang2020local,karimireddy2022byzantinerobust,li2023experimental}, the presence of data heterogeneity imposes additional challenges on the exclusion of the influence of malicious updates in FL. Higher levels of data heterogeneity result in increased diversity in the local updates, making it more challenging to identify and exclude the effects of malicious updates.

% Specifically, heightened levels of heterogeneity amplify the diversity of local updates, thereby complicating the defenses of identifying and excluding the effects of malicious updates.  


% \myparatight{Local Steps} 

% \input{pipeline}

==> tables/background.tex <==

\section{Background}
    \subsection{FL and Optimization}
	\label{sec_formulation}

In FL, a collection of clients collaboratively learn a shared global model using their private datasets in a distributed manner, assisted by the coordination of a central server. The goal is to find a parameter vector $\bm{w}$ that minimizes the following distributed optimization model:
	\begin{equation}
		\label{obj}
		\min\limits_{\bm{w}} F(\bm{w}) :=  \frac{1}{K} \sum_{k \in [K]}  F_k(\bm{w}),
	\end{equation}
	where $K$ represents the total number of clients and $F_k(\bm{w}) = \expect_{\bm{z}\sim \mathcal{D}_k} [\loss(\bw; \bm{z})]$ denotes the expected risk of the $k$-th client. Here,
    $\mathcal{D}_k$ is the data distribution for the $k$-th client 
	and $\loss(\cdot;\cdot)$ is a user-specified loss function.
% 	For each $k$ and $\bm{w}$, we assume $g_k( \bm{w})$ is an unbiased stochastic gradient of the client's true gradient $\grad F_k( \bm{w})$.
% 	, $x_{k,j}$ is a training sample, and $n_k$ is the size of training dataset owned by client $k$.


\begin{comment}
	\begin{algorithm}[!ht]
		\algdef{SE}[SUBALG]{Indent}{EndIndent}{}{\algorithmicend\ }%
		\algtext*{Indent}
		\algtext*{EndIndent}
		\setlength{\abovedisplayskip}{0pt}
		\setlength{\belowdisplayskip}{0pt}
		\setlength{\abovedisplayshortskip}{0pt}
		\setlength{\belowdisplayshortskip}{0pt}
		\caption{Optimization of FL}
        \begin{flushleft}
        \hspace*{\algorithmicindent} \textbf{Input:} $K, T, \eta_t$, $\bw^{0}$
        \end{flushleft}
		\label{alg}
		\begin{algorithmic}[1]
			\For{each global round $t \in [T]$}
			   \State{Select a subset $S_t$ from $N$ clients at random.}
			\For{each client $k \in S_t$ \textbf{in parallel}}
			\State{$\bm{w}_k^t \leftarrow \bm{w}^t$}
			\For{ $E_l$ local rounds, } \label{ag_g_data}
			\State{Compute an estimate $g_k( \bm{w}_{k} ^ t)$ of $\grad F_k( \bm{w}_{k} ^ t)$}
			\State{$ {\displaystyle \bm{w}_{k} ^ t \leftarrow  \text{CLIENTOPT} (\bm{w}_{k} ^ t, g_k( \bm{w}_{k} ^ t), \eta_l), t}$}
			\EndFor
			\State $\update_k^t \leftarrow \bm{w}_{k}^t - \bm{w}^t$ \label{update_cal}

			\State{Sends $\Delta_k^t$ back to the server} \label{ag_g_update}
			\EndFor
			\State $\Delta^{t+1} \leftarrow \text{AGG}(\{\Delta_k^t\}_{k\in [K]})$

			\State $\bm{w}^{t+1} \leftarrow \text{SERVEROPT}(\bm{w}^{t}, -\Delta^{t+1}, \eta_g, t)$
			\EndFor
			\State \Return $\bw^{T}$
		\end{algorithmic}
		\label{opt}
	\end{algorithm}
\end{comment}

% \begin{comment}
\begin{algorithm}[t]
    \algdef{SE}[SUBALG]{Indent}{EndIndent}{}{\algorithmicend\ }%
    \algtext*{Indent}
    \algtext*{EndIndent}
    \setlength{\abovedisplayskip}{0pt}
    \setlength{\belowdisplayskip}{0pt}
    \setlength{\abovedisplayshortskip}{0pt}
    \setlength{\belowdisplayshortskip}{0pt}
    \caption{A \fedavg-family Algorithm for FL}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input:} $K, T$, $\bw^{0}$, CLIENTOPT, SERVEROPT
    \end{flushleft}
    \label{alg}
    \begin{algorithmic}[1]
        \For{each global round $t \in [T]$}
        \State{Select a subset $S_t$ from $K$ clients at random}
        \For{each client $k \in S_t$ \textbf{in parallel}}
        \State{$\bm{w}_k^t \leftarrow \bm{w}^t$}
        \For{$E_l$ local rounds} \label{ag_g_data}
        \State{Compute an estimate $g_k( \bm{w}_{k} ^ t)$ of $\grad F_k( \bm{w}_{k} ^ t)$}
        \State{$ {\displaystyle \bm{w}_{k} ^ t \leftarrow  \text{CLIENTOPT} (\bm{w}_{k} ^ t, g_k( \bm{w}_{k} ^ t), \eta_l, t)}$}
        \EndFor
        \State $\update_k^t \leftarrow \bm{w}_{k}^t - \bm{w}^t$ \label{update_cal}

        \State{Send $\Delta_k^t$ back to the server} \label{ag_g_update}
        \EndFor
        \State $\Delta^{t+1} \leftarrow \text{AGG}(\{\Delta_k^t\}_{k\in [K]})$

        \State $\bm{w}^{t+1} \leftarrow \text{SERVEROPT}(\bm{w}^{t}, -\Delta^{t+1}, \eta_g, t)$
        \EndFor
        \State \Return $\bw^{T}$
    \end{algorithmic}
    \label{opt}
\end{algorithm}
% \end{comment}

The most popular algorithms in the literature that solve \eqref{obj} are the \fedavg-family algorithms~\cite{mcmahan2017communication,reddi2020adaptive,ju2023accelerating}. As shown in Algorithm~\ref{alg}, at $t$-th round of communication, a subset of clients $S_t$ is selected, typically through a random sampling process. The server then broadcasts its current global model parameters $\bm{w}^t$ to each of the selected clients. Simultaneously, the clients independently perform local optimization on their respective private data, aiming to minimize their own empirical loss. This process involves multiple local rounds, denoted as $E_l$, where the clients compute an estimate $g_k(\bm{w}_k^t)$ of the gradient $\nabla F_k(\bm{w}_k^t)$ using their local data. The client model's $\bm{w}_k^t$ are iteratively updated using the estimated gradient and a client-specific learning rate $\eta_l$. The computed local model updates, denoted as $\update_k^t$, are then transmitted back to the server. The server aggregates these updates using an aggregation rule, often averaging aggregation~\cite{mcmahan2017communication}, to generate a global update. This update represents a direction for the global optimizer, capturing the collective knowledge of the participating clients. Subsequently, the server employs the global optimizer, denoted as $\text{SERVEROPT}$, to update the global model's parameters $\bm{w}^t$ using the negative of the aggregated updates, denoted by $-\update_k^{t+1}$ (which is called ``pseudo-gradient''~\cite{reddi2020adaptive}), and a global learning rate $\eta_g$. By iterating this process for multiple rounds, the \fedavg-family algorithms refine the global model through leveraging the distributed computing capabilities and decentralized datasets of the participating clients.

In alignment with previous research~\cite{liconvergence}, we adopt the full client participation strategy in this paper. Therefore, all clients are actively engaged at each training round, which means that $|S_t| = K$ in Algorithm~\ref{alg}.  The rationale behind this choice is grounded in a prevailing assumption of Byzantine-resilient studies in FL, i.e., the number of malicious updates for aggregation is less than half during each round. Selecting subsets at random violates this assumption by chance, as it may select more malicious clients than benign ones by chance~\cite{li2023experimental}. 
% $CLIENTOPT$ minimizes \eqref{obj} based on each client's local data using a local learning rate $\eta_l$ while $SERVEROPT$ aims to optimize from a global perspective using a global learning rate $\eta_g$.

% 	To solve a federated optimization problem, general solvers

	% 	We highlight the following representative attacks:


% 	\subsection{FL Simulators}
%     Recently, several frameworks have been proposed for FL simulations,  including~\cite{beutel2020flower}

\subsection{Byzantine Attacks and Defenses in FL}

Byzantine attacks pose a significant threat to FL due to its distributed optimization nature~\cite{lyu2020threats,rodriguez2023survey}.  
In general, the malicious clients may upload arbitrary parameters to the server to degrade the global model's performance. Hence, in Algorithm~\ref{alg}, the \fedavg-family algorithm we consider in this work, Line~\ref{update_cal} can be replaced by the following update rule:
	\begin{align}
		\label{inner_solution}
		\update_k^t &\leftarrow
		\begin{cases}
			\star            & \text{if $k$-th client is Byzantine,} \\
			\bm{w}_{k}^t - \bm{w}^t & \text{otherwise,}
		\end{cases}
	\end{align} where $\star$ represents arbitrary values.


% We focus on untargeted Byzantine attacks where the adversary's goal is to minimize the accuracy of the global model on any test input~\cite{baruch2019little,fang2020local,shejwalkar2021manipulating,li2023experimental}. Assuming different levels of the adversary's capabilities and knowledge, many attack strategies have been presented to investigate the security threats of FL~\cite{pmlrv139karimireddy21a,li2019rsa,baruch2019little,shejwalkar2021manipulating}. For instance, with minimal capability and knowledge, the adversary can modify a single client's input and output data without access to the training pipeline; some advanced attacks assume the adversary with full knowledge of the learning system to tailor an attack strategy bypassing the defenses. 

% the above paragraph duplicates the following one

As aforementioned, the focus of this work is on untargeted Byzantine attacks, where the adversary's objective is to minimize the accuracy of the global model for any test input~\cite{baruch2019little,fang2020local,shejwalkar2021manipulating,li2023experimental}. Various attack strategies have been proposed to explore the security vulnerabilities of FL, taking into account different levels of the adversary's capabilities and knowledge~\cite{pmlrv139karimireddy21a,li2019rsa,baruch2019little,shejwalkar2021manipulating}. For instance, with limited capabilities and knowledge and without having access to the training pipeline, the adversary can manipulate a single client's input and output data. In more sophisticated attacks, the adversary possesses complete knowledge of the learning system and designs attack strategies to circumvent defenses. Regarding defenses, robust aggregation rules are widely employed to enable Byzantine-resilient estimation of the true updates and mitigate the influence of malicious updates \cite{blanchard2017machine,yin2018byzantine,chen2017distributed,li2021byzantine,karimireddy2021learning,sattler2020byzantine}. Furthermore, other research directions such as trust-based strategies \cite{cao2021fltrust,9887909,sageflow} and variance-reduced algorithms \cite{gorbunov2023variance,9153949} are also worth investigating. For a detailed exploration of the core techniques and aspects of Byzantine attacks and defenses in FL, we refer to Section~\ref{attack_defense_sec}.

% As for defenses, robust aggregation rules are widely applied to make a Byzantine-resilient estimation of the true updates and exclude the influence of malicious updates~\cite{blanchard2017machine,yin2018byzantine,chen2017distributed,li2021byzantine,karimireddy2021learning,sattler2020byzantine}. Furthermore, other directions of studies, such trust-based strategies~\cite{cao2021fltrust,9887909,sageflow} and variance-reduced algorithms~\cite{gorbunov2023variance,9153949} also worth to investigate. We refer to Section~\ref{attack_defense_sec} for the core techniques and aspects of Byzantine attacks and defenses in FL. 
	% In naive \fedavg-family algorithms, Byzantine clients can modify the mean of the updates to their desired direction~\cite{li2021byzantine}. Byzantine attacks can be categorized into targeted attacks and untargeted attacks~\cite{jere2020taxonomy,lyu2020threats}. Targeted attacks, such as backdoor attacks, strive to make the global model misclassify some particular test samples~\cite{xie2019dba,bagdasaryan2020backdoor,andreina2021baffle}, while untargeted attacks aim to degrade the overall performance of the global model indiscriminately~\cite{fang2020local}. Although different robust aggregation schemes have been proposed to mitigate the impact of the malicious behaviors~\cite{chen2017distributed,blanchard2017machine,yin2018byzantine}, the robustness is typically based on strong assumptions on the variance of the updates, which are often violated in practice. Moreover, the field is yet to be explored to defend against new types of attacks.
 
\subsection{Connecting Byzantine-resilient FL with Traditional Distributed Learning }

The study of Byzantine-resilient FL has its roots in the realm of traditional distributed learning, where a central server distributes data to workers who perform gradient estimation; the gradients are then collected and aggregated by the server for model update~\cite{ alistarh2018byzantine,yin2018byzantine,chen2017distributed}. FL originally emerged as an extension of distributed learning to address the limitations imposed by communication constraints and privacy concerns associated with decentralized data ownership~\cite{yin2021comprehensive}. Although FL and traditional distributed learning are employed in different application domains~\cite{li2020review}, they face similar security vulnerabilities stemming from Byzantine attacks due to the distributed nature of optimization. Furthermore, many existing techniques initially proposed for studying Byzantine-resilient distributed learning~\cite{blanchard2017machine,chen2017distributed,yin2018byzantine,bernstein2018signsgd,baruch2019little} have now found extensive application in the defense mechanisms utilized in FL~\cite{pillutla2019robust,fang2020local,shejwalkar2021manipulating,9833647,li2022experimental}. Therefore, it is important to examine FL and traditional distributed machine learning together when it comes to Byzantine resilience.

Benefiting from the generality of Algorithm~\ref{alg}, obtaining traditional distributed learning algorithms is straightforward. For example, by assuming both ``CLIENTOPT'' and ``SERVEROPT'' as a gradient descent step and setting $E_l=1$ and $\eta_l=1$, Algorithm~\ref{alg} simplifies to the naive distributed SGD with gradient aggregation~\cite{chen2017distributed}. In contrast, setting $\eta_g=1$ leads to the naive \fedavg algorithm. This connection enables the generalization of traditional techniques, such as robust aggregation rules, from traditional distributed learning to suit the requirements of FL.


\subsection{Simulators for FL}

    In FL, simulators can provide a fast evaluation of a particular solution's potential utility and help investigate novel approaches before making real deployments. Recently, several FL simulators have been proposed with different foci and scopes. For example, LEAF~\cite{caldas2018leaf} provides open-source federated datasets and metrics for evaluation; PrivacyFL~\cite{mugunthan2020privacyfl} and Pysyft~\cite{ziller2021pysyft} focus on the privacy guarantees of FL algorithms. FLUTE~\cite{dimitriadis2022flute} is designed for optimization and high-performance simulation of FL. However, there is a lack of focus on the simulation of robustness and security concerns. To fill in this gap, we have developed \ours.

==> tables/blades.tex <==
\begin{figure}[ht]
	\centering
	\includegraphics[width=.95\linewidth]{./figs/arch_v2}
	\caption{Illustration of our three-layer architecture for \ours. The application layer facilitates specific FL algorithms with attacks and defenses implementation. The execution layer provides a scalable backend for distributed training. The data layer manages training data retrieval and preprocessing operations.
	}
	\label{arch}
\end{figure}


\section{The Design of \ours}
\label{sec_design}
% In this section, we first introduce the system design of \ours. Then, we highlight some key features of \ours. Finally, we give an example to demonstrate the ease of use to run experiments with the simulator.
In this section, we introduce the \ours simulator, which facilitates researchers and developers to benchmark adversarial FL training and evaluate performance efficiently.

\subsection{Design Goals}
 \ours is a unified benchmark suite designed for simulating various Byzantine attacks and defense strategies in FL. 
The architecture of \ours is carefully designed to address the following key objectives:

\myparatight{Specificity} Different from existing FL simulators~\cite{mugunthan2020privacyfl, dimitriadis2022flute,ziller2021pysyft}, \ours is specifically designed to simulate attacks and defenses. Thus, we should provide built-in implementations of representative attack strategies and robust aggregation schemes so that end users can efficiently validate their approaches and compare them with existing solutions.

\myparatight{Scalability} A benchmark suite for FL must exhibit scalability in terms of both clients and computing resources. 
Scalability with clients refers to the ability to accommodate a large and diverse set of clients participating in the learning process. Scalability with computing resources entails efficiently utilizing and adapting to different computational setups.
% This is crucial as federated learning involves a massive number of clients, ranging from thousands to millions. Similarly, scalability with computing resources involves handling the computational demands of federated learning algorithms, including model training, aggregation, and communication tasks. A scalable benchmark suite efficiently utilizes available computing resources and adapts to varying levels of computational capabilities. By incorporating scalability in these aspects, the benchmark suite enables realistic and comprehensive evaluations of federated learning approaches across different scales and deployment scenarios. It aids researchers and practitioners in analyzing algorithm scalability and performance under various conditions, facilitating the development and optimization of federated learning techniques for real-world applications. In resource-constrained systems, \ours allows each trainer/actor to deal with multiple clients' requests sequentially; thus, the scale of experiments is not limited by the number of workers. Based on Ray, \ours is deployable either on a single machine or a computing cluster. Given that real-world FL would encounter a large number of clients, \ours should scale to a large number of concurrent clients to foster research on a realistic scale. 

\myparatight{Extensibility} \ours should support FL configurations of different models, datasets, and optimizers, including standardized implementations such as \fedsgd and \fedavg. The PyTorch framework has been selected as the preferred choice for implementing the models.  \ours should also allow end users to incorporate new types of attacks, defenses, and optimization algorithms easily.
% with Pytorch being the framework of choice for implementing the models.

\subsection{Core Framework Architecture}
To achieve the design goals, especially regarding scalability and extensibility, we decompose the system into three distinct layers: the Application layer, Execution layer, and Data layer. An overview of the architecture of our \ours is illustrated in Fig.~\ref{arch}. The rationale behind this design is to separate the design goals and foster a modular architecture, thereby enabling optimizations tailored to the specific requirements of each goal. The Application layer focuses on providing extensibility, allowing for easy configuration and integration of various FL-related functionalities and features. The Execution layer is responsible for ensuring the scalability of the system, enabling efficient handling of large workloads and resources. Furthermore, the Data layer functions as an auxiliary component, aiming at enhancing data loading and pre-processing in the distributed environment.

\subsubsection{Application Layer}
It is the top layer of \ours and provides a user-friendly interface for designing and deploying FL algorithms. The main abstractions in this layer include:

\myparatight{Server} A server is an object that aggregates model updates from multiple clients and performs global optimization. Once a local training round is finished, it gathers the model updates and takes one iteration step.  Defense strategies, such as robust aggregations, are usually applied here to eliminate the impact of malicious updates.

\myparatight{Trainer} The trainer encapsulates the optimization process for a particular FL algorithm. A trainer is responsible for managing key aspects of the training loop, including interactions with the server, client group management, and state synchronization between the server and clients. Each trainer corresponds to a specific FL algorithm, such as \fedavg, and can be configured with various hyperparameters to control the local training process. It also allows customization  with callbacks invoked at specific points during training, such as after each local training round or server optimization step. The ``Adversary'' component in the Trainer can control a subset of clients to perform malicious operations.

\myparatight{Client} The client acts as a participant in the FL process. We provide the client-oriented programming design pattern~\cite{he2020fedml} 
% \tv{explain this pattern to make the paper self-contained. Readers do not want to look up other work}
to program the local optimization of clients during their involvement in training or coordination within the FL algorithm. This pattern allows end users to specify and execute certain types of attacks easily. Other than that, users can also customize the behaviors of Byzantine clients using the interface we provide.

\begin{figure}[!t]
\begin{subfigure}[b]{\linewidth}
  \begin{lstlisting}[
language=Python,
linewidth=0.99\linewidth,
]
fedavg_blades:
  run: FEDAVG_DP
  stop: training_iteration: 2000

  config:    
    global_model: resnet
    num_malicious_clients:
      grid_search: [0, 3, 6, 9, 12]
      
    client_config:
      lr: 1.0

    server_config:
      aggregator:
        grid_search: [Mean, Median, GeoMed]

      optimizer:
        type: SGD
        lr: 0.1
        lr_schedule: [[0, 0.1], [1500, 0.1]]
        momentum: grid_search: [0.0, 0.5, 0.9]

    adversary_config:
      grid_search:
        - type: LabelFlipAdversary
        - type: IPMAdversary
            scale: 0.1
\end{lstlisting}
    \end{subfigure}
\caption{\small An example configuration file for simulating the LableFlipping attack~\cite{li2023experimental} and IPM attack~\cite{baruch2019little}. \ours is fully configurable and allows grid search for hyperparameter tuning.}
\label{config_code}
\end{figure}

The application layer has several dependencies that provide a variety of functionalities. Particularly, we adopt the Tune library\footnote{\url{https://docs.ray.io/en/latest/tune}}~\cite{liaw2018tune} for experiment configuration and hyperparameter tuning at any scale. As an example, Fig.~\ref{config_code} shows a configuration file for simulating the LableFlipping~\cite{li2023experimental} and IPM~\cite{baruch2019little} attack with different hyperparameter settings. With the help of Tune, \ours can read the file and parse the configurations to generate a series of experimental trials. The trials are then scheduled to execute on the execution layer. Notably, the ``\code{grid\_search}'' keyword allows for the different combinations of hyperparameters and configurations in the grid, containing ``\code{num\_malicious\_clients}'', ``\code{server\_config}'', and ``\code{adversary\_config}'' in this example, which results in 90 trails at once.

\subsubsection{Execution Layer} 

\input{execution_layer}




\subsubsection{Data Layer} The data layer facilitates data pre-processing and loading for distributed training with the execution backend. It supports both IID and Non-IID partitions for studying homogeneous and heterogeneous scenarios, respectively. At the beginning of the training, the dataset is separated into multiple shards and pre-allocated to workers' memory to allow fast data loading. In addition, we provide adapters to import datasets from well-known 3rd-party benchmarks in FL, such as LEAF~\cite{caldas2018leaf}, FedML~\cite{he2020fedml}, and TensorFlow Federated~\cite{abadi2016tensorflow}.



\begin{comment}
 The %backend layer
 backend of \ours offers two training modes, trainer mode, and actor mode, to meet the different needs of distributed simulations. The trainer mode creates one Ray trainer object for each client. The trainers distributed actor groups for Distributed Data-Parallel Training (DDP), i.e., the global model is replicated on every process, and every model replica will be fed with a different set of input data samples. DDP takes care of gradient communication to keep model replicas synchronized and overlaps it with the gradient computations to speed up training. The actor mode, on the other hand, initializes Ray actors to handle local optimization for each client independently. \tv{I agree with Edith's comments}


The backend of \ours offers two training modes, actor mode and trainer mode, to meet the different needs of the simulations. The actor mode creates a fixed number of Ray actors and uniformly distributes computing resources to all Ray actors. Local training tasks of all clients are evenly divided and assigned to Ray actors. This mechanism enables scalability in terms of variable numbers of clients with fixed computing resources. In order to simulate the resource heterogeneity of federated learning, the trainer mode is introduced. The trainer mode creates one Ray trainer object for each client, which can contain variable Ray actors even across different nodes. The trainer mode enables Distributed Data-Parallel Training (DDP) for local training and flexible resource configurations of each individual client.





\subsection{Communication Layer}
For single GPU and CPU systems, the model parameters are communicated between processes (e.g., actors and the server) via the Inter-Process Communication (IPC) mechanism provided by CUDA. Specifically, processes can move their data into a shared memory block and only send a handle to another process. This mechanism can dramatically reduce communication time, especially for large neural networks.

For Multi-GPU and Multi-Machine systems, \ours uses the distributed package included in PyTorch (i.e., torch.distributed), to speed up the computations across processes and clusters of machines. The distributed package offers a set of native collective primitives for communication between distributed CPUs or GPUs. By default, the server uses the ``gather'' primitive to collect local updates and ``broadcast'' to broadcast the global model to actors.

\end{comment}
% Upon the backend, \ours consists of a collection of clients and a parameter server. In each round of local optimization, each selected client receives the global model from the parameter server and acquires a trainer/actor to perform local training using its private dataset. %In this layer, w


% the honest clients can strictly follow the same updating rules by default (e.g., local SGD), while

% The parameter server plays the role of the defender, which strives to limit the potential influence of the attackers and updates the global model in a robust manner. \ours provides the latest robust aggregation schemes as the build-in defense mechanisms, including \gm~\cite{chen2017distributed}, \krum~\cite{blanchard2017machine}, \tm~\cite{yin2018byzantine}, and  \median~\cite{yin2018byzantine}. In addition, we also provide user-friendly interfaces for the customization of new defense mechanisms.

\subsection{Implementation of Attacks and Defenses using \ours} 


\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{./figs/client_pipeline}
	\caption{\small The pipeline for implementing attacks using \ours. We define some time points when
users can register executable methods to perform customized attacks. At specific time points, client callbacks and adversary callbacks are triggered to invoke the registered methods.}
	\label{pipeline}
\end{figure}


% The optimization processes of FL tasks typically follow a similar workflow. A central server broadcasts a global model to clients to enable local training. The clients, in their turn, update the global model with several steps of SGD using local datasets, and send the updates back to the server. After receiving local updates, the server will aggregate them, typically into a single global model.

The optimization processes in FL tasks typically follow a similar workflow. A central server broadcasts a global model to participating clients, who perform local training using their own datasets. The clients then send their model updates back to the server, which aggregates them into a new global model. This iterative process continues until the desired level of model performance is achieved.


\subsubsection{Implementing Attacks}
We note that adversarial attackers may perform some self-defined manipulation before or after specific time points. For instance, LabelFlipping~\cite{pmlrv139karimireddy21a} attacks are typically executed at the beginning of batch forward propagation, while SignFlipping~\cite{li2019rsa} attacks are carried out immediately after backpropagation. To address this, we have designed a unified pipeline integrated with a callback mechanism, which enables actions to be performed at various stages of training, as depicted in Fig.~\ref{pipeline}. A callback or callback method is any reference to executable code that is passed as an argument to another piece of executing code. The callback method is expected to execute at some defined time points.


This design offers extensibility to facilitate customization, where the minimal pipeline focuses on repetitive local training and server-side optimization while the malicious behaviors are defined through the callback mechanism. Users only need to override specific callback methods to execute a custom attack without modifying the pre-defined logic.

The pipeline consists of two levels of callbacks: client level and adversary level. Since the attacks at Levels 1 \& 2 only have access to local model parameters and datasets, they can be easily implemented by registering behaviors to the client objects and hereby can be executed in parallel on multiple nodes or cores. As an illustrative instance, the upper panel of Fig.~\ref{atk_sim_code} shows a code snippet that exemplifies the implementation of a LabelFlipping attack on a classification task encompassing 10 distinct classes. Through a straightforward customization of the "\code{on\_batch\_begin()}" callback method, the user can effortlessly modify the labels from class $i$ to $9-i$ during local training. 
% To further demonstrate the simplicity of assessing contemporary attacks and strategies within the context of FL, we present additional examples in the Appendix.

For attacks at Level 3 and above, clients in the distributed environment need to exchange data, coordinate actions, and synchronize their activities for making decisions regarding malicious actions. A straightforward solution to simulate such attacks is allowing inter-client communication using the remote function mechanism in Ray. However, this will make the simulation more complex and limit the scalability of the system. One possible consequence is the occurrence of deadlocks~\cite{holt1972some}, i.e., when two or more clients are waiting for each other to release a resource or respond to a communication, none of them can proceed. 

Alternatively, our \ours facilitates the implementation of sophisticated attacks by incorporating supplementary callbacks tailored for adversary entities. Distinguished from client callbacks, these adversary callbacks are executed within the driver program and allow convenient access to various system components and their states. As a result, this design simplifies the process of acquiring knowledge for high-level attacks. Fig.~\ref{pipeline} also shows two of the most essential adversary callbacks, specifically ``\code{on\_algorithm\_begin()}'' and ``\code{on\_local\_round\_end()}''. The former is triggered at the start of the algorithm and serves the purpose of initializing the adversary and setting up client callbacks. The latter is triggered upon the completion of a local round and allows for the modification of collected updates from malicious clients before proceeding to server-side optimization and defense operations. During the ``\code{on\_local\_round\_end()}'' callback, one can potentially access honest updates and other system states in a read-only manner to launch omniscient attacks (Levels 4 \& 5). The lower panel of Fig.~\ref{atk_sim_code} shows an example of implementing the ALIE~\cite{baruch2019little} attack using the proposed callback method. 

\begin{figure}[!t]
\begin{subfigure}[b]{\linewidth}
  \begin{lstlisting}[
    language=Python,
    linewidth=0.99\linewidth,
    ]
from blades.clients import ClientCallback

class LabelFlipCallback(ClientCallback):
    def on_batch_begin(self, data, target):
        # This method returns original input data with flipped labels for the current batch (assuming 10 labels).
        return data, 9 - target
\end{lstlisting}
\vspace{-3pt}
\end{subfigure}

\begin{subfigure}[b]{\linewidth}
  \begin{lstlisting}[
language=Python,
linewidth=0.99\linewidth,
]
from blades.adversary import AdversaryCallback

class ALIECallback(AdversaryCallback):
    def on_local_round_end(self, trainer):
        # This method computes the dimensional mean and std over client updates, then sets the malicious updates within the range of std.
        updates = trainer.get_updates()
        mean = updates.mean(dim=0)
        std = updates.std(dim=0)

        updates_m = mean + std
        trainer.save_malicious_updates(updates_m)
\end{lstlisting}
    \end{subfigure}
\caption{\small Illustration of our callback mechanism for simulating the LableFlipping attack (upper)~\cite{li2023experimental} and ALIE attack (lower)~\cite{baruch2019little}. The flexibility of our design allows for convenient customization through the overriding of respective methods of client callbacks and adversary callbacks.}
\label{atk_sim_code}
\end{figure}


% which are triggered at the beginning of the algorithm and upon the completion of a local round, respectively. ``\code{on\_algorithm\_begin()}'' is not only used to set up the adversary itself, but is also used to set up client callbacks. Before proceeding to the server-side optimization and defense operations, one can modify the collected updates of malicious clients through ``\code{on\_local\_round\_end()}'', possibly with read-only access to honest updates and other states of the system. 

\subsubsection{Implementing Defenses}
As emphasized in Section~\ref{sec_defense}, defenses in the context of our study stem from multiple facets, posing challenges to the establishment of a standardized pipeline akin to the one employed for attacks. Nevertheless, certain indispensable steps are involved in this process, namely update aggregation and global model optimization, although the specific methodology for each step may vary. The update aggregation step combines the locally collected updates, while the global model optimization step performs an optimization procedure based on the aggregated result.

 As such, \ours introduces a foundational abstraction of the server entity, encompassing essential components such as a global model, an aggregator, and an optimizer. This architecture permits the extension of functionalities through the utilization of sub-classing, thereby facilitating the integration of advanced features.  It is noteworthy to mention that even in the minimal server implementation, we offer a configurable SGD optimizer and a variety of pre-defined robust aggregation rules. Furthermore, all the components are modularized and inheritable, allowing plug-and-play of different configurations. We believe our designs can simplify the process of generating benchmark results with minimal effort.
 
% \subsection{Implications of \ours}

==> tables/classic_agr.tex <==

\newcommand \rot{90}
\newcommand{\rotbox}[1]{\rotatebox[origin=c]{0}{#1}}
\begin{table*}[]
\setlength\extrarowheight{3pt}
\begin{adjustbox}{width=0.95\textwidth,center}

\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|}

\hline

\multirow{2}{*}{Technique Type} &  \multirow{2}{*}{Approach} & \multicolumn{9}{|c|}{Machanisms}  & \multirow{2}{*}{Description} \\
 \cline{3-11}
 &   & \rotbox{Dimension-wise} & \rotbox{Euclidean Distance} & \rotbox{Cosine Distance} & \rotbox{Eigenvector} & \rotbox{Clipping} & \rotbox{Client Blocking} & \rotbox{Momentum} &  \rotbox{Sign-based} &  \rotbox{\makecell{Computation \\  at Server}}  & \\
\hline
\hline %\cline{1-13}
 \multirow{5}{*}{\makecell{Robust Gradient  \\ Aggregation}}   &      Krum~\cite{blanchard2017machine}, Multi-Krum~\cite{blanchard2017machine}     &                    & \checkmark  &  &  &  &  & &  &  & \\
  \cline{2-12}
& GeoMed~\cite{chen2017distributed}   & & \checkmark  &     &  &  & & & &  &\\
 \cline{2-12}
 &  Median~\cite{yin2018byzantine}             & \checkmark                    &               &     &                 &          &           &              &            &  & \\
 \cline{2-12}
& TrimmedMean~\cite{yin2018byzantine}     & \checkmark                    &                    &     &            &          &          &              &            &  & \\  \cline{2-12} 
     &  SignSGD-MV~\cite{bernstein2018signsgd}      & \checkmark                    &          &          &                 &          &                 &              & \checkmark      &  & \multirow{1}{*}{Communication efficient} \\
      % \cline{2-12}
%     & SignSGD-EC~\cite{sohn2020election}       & \checkmark                    &               &     &                 &          &                 &               & \checkmark        & \checkmark   &   &   \\
\hline  % \cline{1-13}
 \multirow{7}{*}{\makecell{Extended Robust \\ Aggregation}} &    Signguard~\cite{xu2022byzantine}            &                       &                    &         &        & \checkmark      &                 &                      & \checkmark      & & \\
       \cline{2-12}
&   RAGE~\cite{data2021byzantine}           &                          &                    &     &    \checkmark        &       &                 &                   &       & & \\
      \cline{2-12}
 &    DnC~\cite{shejwalkar2021manipulating}         &                        &                    &     &    \checkmark        &       &           &              &       & & \\
       \cline{2-12}
&   AutoGM~\cite{li2021byzantine}            &                    &             \checkmark       &    &             &       &                 &                 &       & & \\
       \cline{2-12}
&   MAB-RFL~\cite{wan2022shielding}            &                    &                &  \checkmark   &             &       &        \checkmark          &   &       & & \\
 \cline{2-12}
 &  Clustering~\cite{sattler2020byzantine}            &                          &                    &   \checkmark  &            &       &        &              &       & & \\
      \cline{2-12}
  &   ClippedClustering~\cite{li2023experimental}            &                        &                    &   \checkmark  &            &   \checkmark    &                 &               &              &       &  \\
\hline % \cline{1-13}
\multirow{3}{*}{\makecell{Weight Aggregation}} & RFA~\cite{pillutla2022robust}            &                     &             \checkmark       &    &             &       &                 &               &              &       &   \\
      \cline{2-12}
&      AFA~\cite{munoz2019byzantine}            &                 &                   &  \checkmark   &             &       &           \checkmark        &             &              &       &    \\
\hline % \cline{1-13}
        \multirow{2}{*}{\makecell{Client Blocking}} &    AFA~\cite{munoz2019byzantine}            &                 &                   &  \checkmark   &             &       &           \checkmark        &             &              &       &    \\
      \cline{2-12} 
      &   MAB-RFL~\cite{wan2022shielding}            &                    &                &  \checkmark   &             &       &        \checkmark          &                 &       & & \\
      \cline{2-12} 
      &  SafeguardSGD~\cite{allenzhu2021byzantineresilient}           &  &  \checkmark   &     &   &     &      \checkmark     &               &    &  &   \\
      
      \hline
        \multirow{5}{*}{\makecell{Variance Reduction}} &    CC~\cite{pmlrv139karimireddy21a}            &                   &               &     &          &      \checkmark &                  &      \checkmark              &       & & \\
      \cline{2-12}
&          RESAM~\cite{pmlrv162farhadkhani22a,mhamdi2021distributed}            &           &               &     &          &       &                  &      \checkmark        &              &       &    \multirow{2}{*}{Compatible with aggregation rules} \\
 \cline{2-11}
&   BUCKETING~\cite{karimireddy2022byzantinerobust}            &                    &               &     &   &       &                  &      \checkmark         &             &       &  \\
      \cline{2-12}
 &  Byz-VR-MARINA~\cite{gorbunov2023variance}            &                    &               &     &          &       &                  &              &              &       & \\
      \cline{2-12}
 &  Byrd-SAGA~\cite{9153949}            &                   &               &     &          &       &                  &              &              &       &  \\
\hline
\end{tabular}
\end{adjustbox}
\caption{A summary of defense strategies.}
\label{tb_agr}
\end{table*}


==> tables/contents.tex <==

\section{Introduction}

Federated learning (FL)~\cite{mcmahan2017communication,konevcny2015federated} is an attractive learning paradigm to build collaborative machine learning models on distributed data across a multitude of client devices, such as desktops, mobile phones, and IoT devices. The FL process typically involves several iterative steps: Firstly, a central server distributes the current global model to client devices. Subsequently, the clients independently perform one or multiple local steps of stochastic gradient descent (SGD) using their local datasets and transmit the updates back to the server. The server then aggregates these local updates to generate a new global model, which serves as the basis for the next round of training. Such a paradigm allows clients to execute a significant portion of the computation without disclosing their private training data to a centralized entity or one another. Furthermore, FL exhibits improved communication efficiency compared to traditional distributed learning methods ~\cite{arjevani2015communication}, as it capitalizes on multiple local update steps before transmitting the updates~\cite{konevcny2016federated}.

Due to the distributed nature of optimization in FL, it is vulnerable to Byzantine failures~\cite{lyu2020threats,rodriguez2023survey}, wherein certain participants may deviate from the prescribed update protocol and upload arbitrary parameters to the central server. In typical FL algorithms such as FedAvg~\cite{mcmahan2017communication},  the server aggregates the uploaded updates by computing their sample mean and incorporates the result into the global model. However, it is well-known that this approach can be significantly skewed, even with the presence of a single Byzantine client~\cite{li2023experimental}. The server thus requires Byzantine-resilient solutions to defend against malicious clients. Depending on the adversarial goals, Byzantine attacks in FL can be classified into two categories: targeted attacks and untargeted attacks~\cite{jere2020taxonomy,lyu2020threats}. Targeted attacks, such as backdoor attacks, aim to manipulate the global model to generate attacker-desired misclassifications for some particular test samples~\cite{xie2019dba,bagdasaryan2020backdoor,andreina2021baffle}, while untargeted attacks aim to degrade the overall performance of the global model indiscriminately~\cite{fang2020local}. In this work, we focus on untargeted attacks as most Byzantine-resilient studies do~\cite{blanchard2017machine,yin2018byzantine,chen2017distributed,li2021byzantine,karimireddy2021learning,sattler2020byzantine,9833647}. Due to this, ``Byzantine'' refers to ``untargeted Byzantine'' in the rest of this paper, unless specified otherwise.

% In recent years, the security of federated optimization becomes an important concern due to the distributed execution. Adversarial (Byzantine) clients can modify the local updates maliciously %to their desire
% and upload them to the server during training time, posing a serious threat to the convergence of the optimization~\cite{lyu2020threats}.
%\tv{the previous sentence is very long. You may split it into two sentences}

In recent years, the field of FL has seen the emergence of various Byzantine-resilient approaches. These approaches aim to protect distributed optimization from Byzantine clients and assure the performance of the learned models~\cite{rodriguez2022survey, hu2021challenges}. For instance, robust aggregation rules are widely used to estimate the global update from a collection of local updates while mitigating the impact of malicious behaviors. Typical rules include \gm~\cite{chen2017distributed}, \krum~\cite{blanchard2017machine}, \tm~\cite{yin2018byzantine}, and  \median~\cite{yin2018byzantine}. 
Similarly, different attack strategies are emerging, striving to circumvent defense strategies~\cite {baruch2019little, xie2020fall}. For instance, the A Little Is Enough (ALIE) attack can bypass most robust aggregation rules by taking advantage of the empirical variance between clients' updates if such a variance is high enough, especially when the local datasets are not independent and identically distributed (non-IID)~\cite{baruch2019little,li2022experimental}. Thus, defending against adversarial attacks remains an open problem in FL~\cite{kairouz2021advances}.

\begin{comment}
    

Although we acknowledge the importance of eventual real-world experiments in the context of robust federated optimization, here, we focus on simulation as a way to effectively utilize by researchers and developers to study the behaviors of attackers and validate the robustness of defense strategies before building and deploying in the wild. 
\end{comment}


Moreover, the development of a benchmark suite tailored specifically for Byzantine-resilient FL is crucial for facilitating fair performance comparisons and accelerating the evaluation of novel attack and defense mechanisms. While several open-source frameworks have been developed to enable FL simulations~\cite{dimitriadis2022flute,ziller2021pysyft, mugunthan2020privacyfl}, a unified benchmark suite that can capture the characteristics of adversarial settings and fill the requirement of this field is still lacking.

% to facilitate fair comparison and accelerate the evaluation of different techniques. no comprehensive open-source toolbox currently exists to assist researchers and developers in simulating adversarial attacks and defenses. 
% We identify the following gaps in this field:

% \myparatight{Standardized assumptions for fair comparison} 

% \myparatight{Unified benchmark suits} 


% The ultimate goal of our research is to advance the study of Byzantine attacks and defenses in FL. This paper investigates existing techniques and introduces an open-source benchmark suite, \ours, for convenient and fair algorithmic performance comparisons. This suite facilitates the development of FL algorithms and fosters the exploration of novel defenses against Byzantine attacks, driving progress in FL robustness. Specifically, we make the following key contributions in this work:

\textbf{Our work:} Aiming to advance the study of Byzantine attacks and defenses in FL, we conduct a systematic investigation of existing techniques and introduce an open-source benchmark suite, named \ours, which facilitates convenient and fair algorithmic performance comparisons. This suite enables the development of FL algorithms and encourages the exploration of novel defenses against Byzantine attacks, thereby driving progress in FL robustness. Specifically, we make the following key contributions:

\myparatight{A systematic study on the literature} We start by conducting a systematic study on existing Byzantine attacks and defenses in FL and its predecessor, distributed machine learning, to provide a comprehensive overview of the fundamental aspects and techniques in this domain. Specifically, attacks are classified into five levels based on the adversary’s capabilities and knowledge~\cite{9833647}. Defense strategies are primarily categorized into three branches: Robust Aggregation~\cite{blanchard2017machine,chen2017distributed,yin2018byzantine,karimireddy2021learning,sattler2020byzantine,li2021byzantine,li2023experimental}, Trust-based Strategies~\cite{cao2021fltrust,9887909,sageflow}, and Variance-reduced Algorithms~\cite{gorbunov2023variance,9153949}, according to their inherent characteristics. This study enhances our understanding of the landscape surrounding Byzantine resilience and facilitates the identification of effective countermeasures in FL. It also serves as a foundation for inspiring the design of our benchmark suite.

\myparatight{\ours, a benchmark suite}We introduce \ours, an open-source benchmark suite for \textbf{B}yzantine-resilient federated \textbf{L}earning with \textbf{A}ttacks and \textbf{D}efenses \textbf{E}xperimental \textbf{S}imulation, which is specifically designed to fill the need for studying attack and defense problems in FL. \ours is built upon a versatile distributed framework, Ray, enabling effortless parallelization of single machine code across various settings, including single CPU, multi-core, multi-GPU, or multi-node, with minimal configuration requirements. This makes \ours efficient in terms of execution time, as client and server operations are executed in a parallel manner. In addition, \ours provides a wide range of attack and defense mechanisms and allows end users to easily plug in customized or new techniques. We illustrate the user-friendly nature of \ours through examples and validate its scalability with respect to clients and computational resources. The results highlight that \ours can effectively handle large client populations and computational resources.

\myparatight{Comprehensive experimental evaluations} Using \ours, we extensively examine representative defense techniques against state-of-the-art attacks. The results demonstrate that high-level attacks can inflict significant harm on defense strategies, attributable to the heightened capabilities and knowledge possessed by the adversaries in contrast to lower-level attacks. We also explore key factors (e.g., momentum, the degree of Non-IID, and differential privacy (DP)) that have potential influences on Byzantine resilience. The key takeaways from our experiments can be summarized as follows:

\begin{itemize}
    \item Variance-based attacks such as ALIE pose the most substantial challenge to the robust aggregation rules.
    \item Hybrid defense strategies that integrate multiple techniques demonstrate greater promise compared to purebred defenses.
    \item When employed as an auxiliary technique, client momentum confers advantages in defending against ALIE attacks, whereas server momentum tends to exacerbate the vulnerability.
    \item Both the degree of non-IID in the training data and the budget allocated for privacy preservation have a considerable impact on the robustness of defense mechanisms.
\end{itemize}

 \begin{comment}
     
In summary, we make the following research contributions:
\begin{itemize}
    \item We introduce \ours, a scalable, extensible, and easily configurable simulator for studying attacks and defenses in FL environments.
    \item We implement representative attack strategies and the latest robust aggregation schemes for FL, which can accelerate the generation of benchmark results on new types of adversarial attacks and defenses in FL.
    \item Using \ours, we evaluate typical attacks and defenses through comprehensive experiments conducted in different FL settings.
\end{itemize}
 \end{comment}

\input{background}

\input{attacks_and_defense}

\input{blades}

\input{experiments}


\subsection{Scalability Evaluation}

We evaluate the scalability of \ours along two lines: First, we evaluate the running time for a global round with an increasing the number of clients and computing resources.
Second, we evaluate the running time per round with an increasing number of GPUs.
% With fixed resources, \ours can simulate variable numbers of clients in a simulation. 

To assess the scalability with respect to the number of clients, we conduct simulations with a fixed set of resources and vary the number of clients. As shown in Table~\ref{scal_client}, the number of clients increases from 16 to 512, which greatly outnumbers the available CPUs and GPUs. The results show that with a linear increase in the number of clients, the average running time of each global round increases linearly with little standard deviation, indicating the stable and efficient communication and task distribution implementation in \ours.

\begin{table}[ht]
\caption{\small Experiment for client scalability - average and standard deviation of running time per global round with increasing numbers of clients.}
\begin{center}
\setlength\extrarowheight{2pt}
\begin{adjustbox}{width=.9\linewidth,center}
\begin{tabular}{|c||c|c|c|c|c|c|c}
\hline
    \# Clients & 16 & 32 & 64 & 128 & 256 & 512 \\
\hline
    Avg (seconds) & 1.41 & 2.48 & 4.51 & 9.10 & 17.58 & 34.53\\
\hline
    Std (seconds) & 0.05 & 0.07 & 0.11 & 0.18 & 0.38 & 0.73\\
\hline
\end{tabular}
\end{adjustbox}
\label{scal_client}
\end{center}
\end{table}

\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{figs/blades_scalability.pdf}
\caption{\small Experimental results for resource scalability of \ours. Blue: Average time cost per global round decreases with the increase in the number of GPUs. Orange: The speedup increases with the increase in the number of GPUs.}
\label{time_gpu}
\end{figure}

% To evaluate the resource scalability of \ours, a fixed simulation task of 480 clients is defined for \ours to be done on GPUs. 

In order to evaluate the resource scalability of \ours, we design a simulation task involving 480 clients to be executed on GPUs. Fig. \ref{time_gpu} shows the time cost of each global round with different numbers of GPUs and the associated speedups. The time cost for each global round reduces from 82.5s to 49.5s when the number of GPUs increases from 1 to 2, and the time cost reduces more if more GPUs are added. The speedup achieved does not align precisely with the number of GPUs utilized, primarily because FL is not an entirely parallelizable algorithm. Consequently, a substantial portion of serial work, such as the communication of local updates and model aggregation, hinders the potential speedup. Nonetheless, it can be concluded that the increase in computing resources significantly reduces the time cost of the simulation, and \ours is scalable with computing resources.


\input{related_work}

\section{Conclusion and Future Work}

% This paper investigated existing techniques in Byzantine-resilient FL and introduced an open-source benchmark suite to fill the need for studying attack and defense problems in FL. \ours provides scaling capabilities, several state-of-the-art attack and defense strategies, and flexible interfaces enabling the implementation and extension of novel attack and defense strategies. Using \ours, we extensively examined representative defense techniques against state-of-the-art attacks and gained insightful findings about Byzantine-resilient FL.
In this paper, we first investigated the existing methodologies employed in Byzantine-resilient FL. Then we introduced an open-source benchmark suite to address the research gap concerning attack and defense problems in FL. The \ours framework offers scalability, integration of cutting-edge attack and defense strategies, and adaptable interfaces that facilitate the implementation and expansion of novel attack and defense techniques. By utilizing \ours, we conducted a comprehensive evaluation of prominent defense techniques against state-of-the-art attacks, yielding insightful findings regarding the resilience of Byzantine-resilient FL.
% sIn addition to models and tasks, \ours provides facilities for easy integration of arbitrary models and training schemes based on PyTorch. 
% \tv{add the main take-aways here as well}
Furthermore, we validated \ours %with extensive experiments and conclude that 
and showed that \ours is scalable in terms of both the number of clients and computing resources.  
We will continue our efforts to address new challenges with our new releases of \ours. We encourage the research community to explore new research using \ours and invite contributions to the public source repository.
% In the development of \ours, we have identified several key challenges in developing high-performance FL simulators. First, the communication and CPU overhead of managing many client tasks and model updates tends to impose a bottleneck that prevents optimal GPU usage. In addition, the standard model and dataloader APIs require additional wrapper code, which is often task-dependent, to facilitate easy integration into a federated learning framework. We will continue our efforts to address these challenges with new releases of the platform.

% The goal of \ours is to enable rapid experimentation and prototyping and facilitate the development of new research efforts on the robustness of federated learning. We encourage the research community to explore new research using \ours and invite contributions to the public source repository.

%\begin{acks}
% XXX to add for final version
%\end{acks}

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.


==> tables/defense_table.tex <==
% \newcommand \alignline{ \cline{2-11}}
\newcommand \alignline{ }
\newcommand \secondalignline{ \cline{1-11}}
\newcommand \thickvline{ \color{black}\vline width 1pt}
\newcommand{\rotbox}[1]{\rotatebox[origin=c]{85}{#1}}
\begin{table}[!t]
\caption{A summary of robust aggregation rules. Those highlighted in bold will be evaluated through experiments in Section~\ref{sec_exp}.}
\begin{threeparttable}
\setlength\extrarowheight{3pt}
% \vspace*{-.3cm}
\begin{adjustbox}{width=0.99\linewidth,center}

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{c|c|ccccccccc}
\hline
  \textbf{\makecell{Aggregation \\ Type}}& \textbf{Reference}  &  \rotbox{\textbf{Dimension-wise}} & \rotbox{\makecell{\textbf{Euclidean} \\ \textbf{Distance-based}}} & \rotbox{\makecell{\textbf{Cosine} \\ \textbf{Distance-based}}} & \rotbox{\textbf{Eigenvector}} & \rotbox{\textbf{Clipping-Based}} & \rotbox{\textbf{Stateful}} &  \rotbox{\textbf{Sign-based}} &  \rotbox{\textbf{Median-based}}   \\
\hline
\hline
% \secondalignline
  \multirow{5}{*}{\makecell{GAR}}   &      Krum~\cite{blanchard2017machine}, Multi-Krum~\cite{blanchard2017machine}     & & \Checkmark  &  &  &  &  &  &   \\
\alignline
 &\textbf{GeoMed}~\cite{chen2017distributed}   & & \Checkmark & &  &  & & &  \Checkmark \\
\alignline
 &  \textbf{Median}~\cite{yin2018byzantine} & \Checkmark  & & & & & & & \Checkmark   \\
\alignline
& \textbf{Trimmedmean}~\cite{yin2018byzantine} & \Checkmark  & & & &  & & & \\ 
\alignline
     &  SignSGD-MV~\cite{bernstein2018signsgd} & \Checkmark & & & & & & \Checkmark & \\
\secondalignline
 \multirow{8}{*}{\makecell{EGAR}} &    \textbf{SignGuard}~\cite{xu2022byzantine} &   &  & &  & \Checkmark &  & \Checkmark      &   \Checkmark   \\
\alignline

& \textbf{CenteredClipping}~\cite{pmlrv139karimireddy21a} & & & & & \Checkmark &  \Checkmark & &   \\
\alignline
&   RAGE~\cite{data2021byzantine} &   &  & &    \Checkmark &  &  &  &  \\
\alignline
 &    \textbf{DnC}~\cite{shejwalkar2021manipulating}  &  &  & &  \Checkmark & &  &  &   \\
\alignline
&   AutoGM~\cite{li2021byzantine}  &  & \Checkmark  & & & & & &  \Checkmark  \\
\alignline
&   MAB-RFL~\cite{wan2022shielding}& & &  \Checkmark  &  & &\Checkmark & &  \\
\alignline
&  Clustering~\cite{sattler2020byzantine} &&&   \Checkmark  & && & &  \\
\alignline
  &   \textbf{ClippedClustering}~\cite{li2023experimental} & & & \Checkmark  & & \Checkmark   & \Checkmark &&  \Checkmark    \\
\secondalignline
\multirow{2}{*}{\makecell{WAR}} & RFA~\cite{pillutla2022robust} & & \Checkmark &  &  & &  & & \Checkmark  \\
\alignline
&  AFA~\cite{munoz2019byzantine}   & & &  \Checkmark   & & & \Checkmark & &  \\
\alignline
&  RFCL~\cite{alharbi2023robust}   & & &  \Checkmark   & & &  & &  \Checkmark \\
% \Xhline{3\arrayrulewidth}
\hline

\end{tabular}

\end{adjustbox}
%     \begin{tablenotes}
%         {\item [{\color{blue}(*)}] By default, the papers utilize one random sample to estimate gradients, whereas we have opted for a mini-batch version to ensure consistency in our work.}
% \end{tablenotes}
\end{threeparttable}
\label{tb_defense}
\end{table}


==> tables/defense_table_bk.tex <==
\newcommand \alignline{ \cline{2-12}}
\newcommand \secondalignline{ \cline{1-12}}
\newcommand \thickvline{ \color{black}\vline width 1pt}
\newcommand{\rotbox}[1]{\rotatebox[origin=c]{70}{#1}}
\begin{table*}[ht]
\caption{A summary of robust aggregation schemes.}
    \begin{threeparttable}
\setlength\extrarowheight{3pt}
\begin{adjustbox}{width=0.9\textwidth,center}

% \begin{tabular}{!{\color{black}\vline width 1pt}c|c!{\thickvline}c!{\thickvline}c|c|c|c|c|c|c|c!{\color{black}\vline width 1pt}>
% {\columncolor[gray]{0.9}}
% c!{\color{black}\vline width 1pt}l!{\thickvline}}

\begin{tabu}{|c|c|c|c|c|c|c|c[10pt]c|c|c|c|l[1pt]}

% \Xhline{3\arrayrulewidth}
 \multicolumn{1}{|c|}{\textbf{Aggregation Type}} & \textbf{Reference} & \multicolumn{8}{c!{\color{black}\vline width 1pt}}{\textbf{Machanisms}}  &  \\
\hline
\hline
  &  &  \rotbox{Dimension-wise} & \rotbox{\makecell{Euclidean  Distance}} & \rotbox{Cosine Distance} & \rotbox{Eigenvector} & \rotbox{Clipping} & \rotbox{Stateful} &  \rotbox{Sign-based} &  \rotbox{\makecell{Median-based}}  & \rotbox{\makecell{Time \\ Complexity}} \\
% \Xhline{3\arrayrulewidth}

\secondalignline
  \multirow{5}{*}{\makecell{Gradient Aggregation \\ Rules}}   &      Krum~\cite{blanchard2017machine}, Multi-Krum~\cite{blanchard2017machine}     & & \checkmark  &  &  &  &  &  &  & $\mathcal{O}(dn^2) $ \\
\alignline
 &\textbf{GeoMed}~\cite{chen2017distributed}   & & \checkmark & &  &  & & &  \checkmark & $\mathcal{O}(dn \log^3 \epsilon^{-1}) $\\
\alignline
 &  \textbf{Median}~\cite{yin2018byzantine} & \checkmark  & & & & & & & \checkmark  & $\mathcal{O}(dn \log n) $ \\
\alignline
& \textbf{Trimmedmean}~\cite{yin2018byzantine} & \checkmark  & & & &  & & &  & $\mathcal{O}(dn \log n)$ \\ 
\alignline
     &  SignSGD-MV~\cite{bernstein2018signsgd} & \checkmark & & & & & & \checkmark & & $\mathcal{O}(dn)$ \\
\secondalignline
 \multirow{8}{*}{\makecell{Extended Gradient \\ Aggregation Rules}} &    \textbf{SignGuard}~\cite{xu2022byzantine} &   &  & &  & \checkmark &  & \checkmark      &   \checkmark  &  \\
\alignline

& \textbf{CenteredClipping}~\cite{pmlrv139karimireddy21a} & & & & & \checkmark &  \checkmark & & &  \\
\alignline
&   RAGE~\cite{data2021byzantine} &   &  & &    \checkmark &  &  &  & &  \\
\alignline
 &    \textbf{DnC}~\cite{shejwalkar2021manipulating}  &  &  & &  \checkmark & &  &  & &  \\
\alignline
&   AutoGM~\cite{li2021byzantine}  &  & \checkmark  & & & & & &  \checkmark &  $\mathcal{O}(T_g dn \log^3 \epsilon^{-1}) $ \\
\alignline
&   MAB-RFL~\cite{wan2022shielding}& & &  \checkmark  &  & &\checkmark & & &  \\
\alignline
&  Clustering~\cite{sattler2020byzantine} &&&   \checkmark  & && & & & $\mathcal{O}(dn^2  \log n ) $ \\
\alignline
  &   \textbf{ClippedClustering}~\cite{li2023experimental} & & & \checkmark  & & \checkmark   & \checkmark &&  \checkmark   &  $\mathcal{O}(dn^2  \log n ) $ \\
\secondalignline
\multirow{2}{*}{\makecell{Weight Aggregation \\Rules}} & RFA~\cite{pillutla2022robust} & & \checkmark &  &  & &  & & \checkmark  &  $\mathcal{O}(dn \log^3 \epsilon^{-1}) $  \\
\alignline
&  AFA~\cite{munoz2019byzantine}   & & &  \checkmark   & & & \checkmark &&&  \\
% \Xhline{3\arrayrulewidth}
\Xhline{3\arrayrulewidth}
% \hline

% \end{tabular}
\end{tabu}
\end{adjustbox}
%     \begin{tablenotes}
%         {\item [{\color{blue}(*)}] By default, the papers utilize one random sample to estimate gradients, whereas we have opted for a mini-batch version to ensure consistency in our work.}
% \end{tablenotes}
\end{threeparttable}
\label{tb_defense}
\end{table*}


==> tables/defense_table_bk3.tex <==
\newcommand \alignline{ \cline{2-11}}
\newcommand \secondalignline{ \cline{1-11}}
\newcommand \thickvline{ \color{black}\vline width 1pt}
\newcommand{\rotbox}[1]{\rotatebox[origin=c]{70}{#1}}
\begin{table*}[ht]
\caption{A summary of robust aggregation rules. Those highlighted in bold will be evaluated through experiments in Section~\ref{sec_exp}.}
    \begin{threeparttable}
\setlength\extrarowheight{3pt}
\vspace*{-.3cm}
\begin{adjustbox}{width=0.8\textwidth,center}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}

\hline
  \textbf{Aggregation Type}& \textbf{Reference}  &  \rotbox{\textbf{Dimension-wise}} & \rotbox{\makecell{\textbf{Euclidean} \\ \textbf{Distance-based}}} & \rotbox{\makecell{\textbf{Cosine} \\ \textbf{Distance-based}}} & \rotbox{\textbf{Eigenvector}} & \rotbox{\textbf{Clipping-Based}} & \rotbox{\textbf{Stateful}} &  \rotbox{\textbf{Sign-based}} &  \rotbox{\textbf{Median-based}}   \\
\hline
\hline
% \secondalignline
  \multirow{5}{*}{\makecell{Gradient Aggregation \\ Rules}}   &      Krum~\cite{blanchard2017machine}, Multi-Krum~\cite{blanchard2017machine}     & & \checkmark  &  &  &  &  &  &   \\
\alignline
 &\textbf{GeoMed}~\cite{chen2017distributed}   & & \checkmark & &  &  & & &  \checkmark \\
\alignline
 &  \textbf{Median}~\cite{yin2018byzantine} & \checkmark  & & & & & & & \checkmark   \\
\alignline
& \textbf{Trimmedmean}~\cite{yin2018byzantine} & \checkmark  & & & &  & & & \\ 
\alignline
     &  SignSGD-MV~\cite{bernstein2018signsgd} & \checkmark & & & & & & \checkmark & \\
\secondalignline
 \multirow{8}{*}{\makecell{Extended Gradient \\ Aggregation Rules}} &    \textbf{SignGuard}~\cite{xu2022byzantine} &   &  & &  & \checkmark &  & \checkmark      &   \checkmark   \\
\alignline

& \textbf{CenteredClipping}~\cite{pmlrv139karimireddy21a} & & & & & \checkmark &  \checkmark & &   \\
\alignline
&   RAGE~\cite{data2021byzantine} &   &  & &    \checkmark &  &  &  &  \\
\alignline
 &    \textbf{DnC}~\cite{shejwalkar2021manipulating}  &  &  & &  \checkmark & &  &  &   \\
\alignline
&   AutoGM~\cite{li2021byzantine}  &  & \checkmark  & & & & & &  \checkmark  \\
\alignline
&   MAB-RFL~\cite{wan2022shielding}& & &  \checkmark  &  & &\checkmark & &  \\
\alignline
&  Clustering~\cite{sattler2020byzantine} &&&   \checkmark  & && & &  \\
\alignline
  &   \textbf{ClippedClustering}~\cite{li2023experimental} & & & \checkmark  & & \checkmark   & \checkmark &&  \checkmark    \\
\secondalignline
\multirow{2}{*}{\makecell{Weight Aggregation \\Rules}} & RFA~\cite{pillutla2022robust} & & \checkmark &  &  & &  & & \checkmark  \\
\alignline
&  AFA~\cite{munoz2019byzantine}   & & &  \checkmark   & & & \checkmark & &  \\
% \Xhline{3\arrayrulewidth}
\hline

\end{tabular}

\end{adjustbox}
%     \begin{tablenotes}
%         {\item [{\color{blue}(*)}] By default, the papers utilize one random sample to estimate gradients, whereas we have opted for a mini-batch version to ensure consistency in our work.}
% \end{tablenotes}
\end{threeparttable}
\label{tb_defense}
\end{table*}


==> tables/execution_layer.tex <==
The execution backend is built upon a scalable framework Ray\footnote{\url{https://www.ray.io}}~\cite{moritz2018ray} for training and resource allocation. Ray provides two key advantages for \ours: 1) It allows users to customize computing resources (e.g., CPUs and GPUs) to clients and servers conveniently; 2) It enables \ours to easily adapt to in-cluster large-scale distributed training, benefiting from the capabilities of the Ray cluster. The core abstractions in the execution layer are:


\begin{comment}
\myparatight{Worker} A worker is a proxy that can be allocated with computing resources to execute the training pipeline for clients. Inherited from Ray Actor\footnote{\url{https://docs.ray.io/en/latest/ray-core/actors.html}}, the worker (essentially a Python process) is the smallest unit for resource management and distributed computing. In a distributed environment, multiple workers collaborate as a group. In case of a large number of clients and limited resources, multiple clients are mapped to one worker, and their local training tasks will be scheduled to run sequentially. This property enables a much larger scale of experiments on common hardware. Moreover, to maximally utilize resources, actors can request fractional GPUs so that multiple actors can be co-located to the same GPU~\cite{lai2022fedscale}. Such a GPU-sharing technique could accelerate FL optimization for lightweight models.


\myparatight{Worker Manager} The worker manager facilitates a lightweight and efficient mechanism for coordinating worker groups and scheduling tasks within a distributed training environment. It retrieves the training pipelines submitted by clients from a task queue, allocates them to suitable workers, and retrieves results as required.

\myparatight{Object Store Memory} Following the distributed memory management of Ray, \ours allows storing and caching data objects during distributed computations using object store memory. Remote objects are cached in Ray's distributed shared-memory object store, and there is one object store per node in the cluster for easy access. 

\end{comment}

By decoupling the execution layer from the application layer, clients remain unaware of the specific implementation details of the backend. As a result, users can concentrate solely on the application layer for implementing FL algorithms and submitting client training pipelines to the worker group.

==> tables/experiments.tex <==
\begin{figure*}[ht]
	\begin{subfigure}[b]{\linewidth}
		\centering
		\includegraphics[width=\linewidth]{./figs/fashion_mnist}
	\end{subfigure}
	\begin{subfigure}[b]{\linewidth}
		\centering
		\includegraphics[width=\linewidth]{./figs/cifar10}
	\end{subfigure}
% 	\vspace*{-0.5cm}
	\caption{\small Comparing state-of-the-art aggregation rules under various attacks on Fashion MNIST and CIFAR10 datasets with IID partition. Low-level attacks such as LabelFlipping~\cite{pmlrv139karimireddy21a} and Signflipping~\cite{li2019rsa} are ineffective against most of the aggregation rules, while high-level attacks such as ALIE~\cite{baruch2019little} and MinMax~\cite{shejwalkar2021manipulating} result in significant performance degradation across most settings, particularly as the proportion of malicious clients increases. Noticeably, traditional GARs (i.e., \median~\cite{yin2018byzantine}, \tm~\cite{yin2018byzantine}, and \gm~\cite{pillutla2022robust}) exhibit vulnerabilities to several attacks, whereas advanced EGARs display greater resilience against the majority of attacks. }
	\label{atk_sim}
\end{figure*}

\section{Experiments}
\label{sec_exp}
In this section, we first evaluate different built-in attack and defense strategies. We provide new insights into the field of Byzantine-resilient FL by evaluating and comparing existing techniques using \ours.
Then, we test the scalability of \ours in terms of both clients and computing resources.


\subsection{Attacks and Defenses Simulation}

\subsubsection{Experimental Setup}

We simulate an FL system with one server and 60 clients using two popular image classification tasks: Fashion MNIST and CIFAR10. Fashion MNIST~\cite{xiao2017fashion} is a dataset consisting of 50,000 gray-scale training samples and 10,000 test samples. It encompasses 10 different categories of clothing items, such as shoes, T-shirts, and dresses. The images in Fashion MNIST are of size $28 \times 28$. CIFAR10, introduced by Krizhevsky et al.~\cite{krizhevsky2009learning}, is a dataset containing 50,000 color training samples and 10,000 test samples. It comprises color images of various objects classified into 10 categories, including airplanes and automobiles. The images in CIFAR10 have dimensions of $32 \times 32 \times 3$. For Fashion MNIST, we use a five-layer convolutional neural network (CNN). For CIFAR10, we use a lightweight ResNet architecture.
% \tv{motivate why you use these architectures. Easiest with references to other work}

We split each dataset into 60 subsets, following both IID and Non-IID partitions, and allocate them to the clients. For the IID partition, we randomly split the training set into 60 subsets. For the Non-IID partition, we follow prior work~\cite{lin2020ensemble,li2023experimental} and model the Non-IID data distributions with a Dirichlet distribution $\bm{p}_l \sim \textit{Dir}_K(\alpha)$, in which a smaller $\alpha$ indicates a stronger Non-IID data partition. Then we allocate a $\bm{p}_{l,k}$ proportion of the training samples of class $l$ to client $k$.

By default, we repeat each experiment five times with different random seeds for model initialization and evaluate the accuracy of the learned model with a clean test set.

\subsubsection{Robust Aggregation}

\label{sec_agg}
\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{figs/gradient_explosion}
\caption{\small Training loss on Fashion MNIST with noise attacks where $20\%$ of the clients are malicious. We clamp the loss into the range $[0, 10^4]$. Noisy malicious updates lead to gradient explosion, which could be mitigated by gradient clipping and batch normalization.}
\label{gradient_explosion}
\end{figure}



Without loss of generality, we first evaluate the robustness of different aggregation rules using one step of local update, i.e., $E_l = 1$. Fig.~\ref{atk_sim} depicts the overall comparison of the robust aggregation rules with respect to test accuracy under different types of attacks. The results clearly show that the robustness of examined aggregation rules varies depending on the dataset and attack type. Notably, when utilizing the Fashion MNIST dataset, robust aggregation rules maintain higher accuracy compared to CIFAR10, which can be attributed to the relatively lower complexity and diversity  of the Fashion MNIST classification task. 

Regarding the examined attacks, low-level attacks such as LabelFlipping~\cite{pmlrv139karimireddy21a} and Signflipping~\cite{li2019rsa} demonstrate limited effectiveness against most aggregation rules. Conversely, high-level attacks such as ALIE~\cite{baruch2019little} and MinMax~\cite{shejwalkar2021manipulating} lead to substantial performance degradation across various scenarios, particularly with an increased proportion of malicious clients. It should be noted that both ALIE and MinMax leverage the variance of benign updates. However, MinMax typically amplifies the magnitudes to larger values, thereby presenting a mixed set of advantages and disadvantages. On the one hand, larger magnitudes have the potential to push the global model further away if they are not filtered out by the aggregation rules. On the other hand, these amplified magnitudes are more easily detectable by certain defense mechanisms, such as the DnC rule employed in our experiments.

Moving to defenses, traditional GARs (i.e., \median~\cite{yin2018byzantine}, \tm~\cite{yin2018byzantine}, and \gm~\cite{pillutla2022robust}) show vulnerabilities to multiple attack types. As already illustrated in Table~\ref{tb_defense}, these methods rely on either filtering at the dimensional level or optimization based on Euclidean distance, both of which have been deemed insufficient in previous studies~\cite{shejwalkar2021manipulating,li2023experimental}. In contrast, advanced EGARs such as \dnc, \clippedclustering, and \signguard exhibit superior resilience against the majority of attacks. These advanced approaches typically employ hybrid mechanisms that incorporate multiple techniques, enhancing their effectiveness in defending against various attack scenarios.
\vspace*{-.2em}
\begin{mybox}
\paragraphb{(Takeaway)} 1) Variance-based attacks pose the most substantial challenge to the established robust aggregation rules.
2) Hybrid strategies that integrate multiple techniques demonstrate greater promise compared to purebred defense strategies.
\end{mybox}

\begin{table*}
\caption{Test accuracy of CIFAR10 on different momentum settings. The numbers with the highest accuracy are in bold. Client momentum significantly improves the robustness.}
	\begin{center}
	\setlength\extrarowheight{2pt}
	\begin{adjustbox}{width=1.0\linewidth,center}
		\begin{tabular}{|c||c|c|c||c|c|c||c|c|c|}
		    \hline
			 Agg. & \multicolumn{3}{c||}{10\% malicious clients} & \multicolumn{3}{c||}{15\% malicious clients} & \multicolumn{3}{c|}{20\% malicious clients}\\
			 \hline
			  & \makecell{No \\ Momentum} & \makecell{Server \\ Momentum} & \makecell{Client \\ Momentum} & \makecell{No \\ Momentum} & \makecell{Server \\ Momentum} & \makecell{Client \\ Momentum} & \makecell{No \\ Momentum} & \makecell{Server \\ Momentum} & \makecell{Client \\ Momentum}\\	
			\hline
\mean~\cite{mcmahan2017communication} & 86.05 (0.20) & 88.46 (0.24) & \textbf{89.51 (0.22)} & 82.89 (0.46) & 80.72 (0.53) & \textbf{88.18 (0.34)} & 73.50 (0.91) & 59.92 (1.36) & \textbf{85.88 (0.22)}\\
\dnc~\cite{shejwalkar2021manipulating} & 85.84 (0.19) & 87.92 (0.45) & \textbf{89.40 (0.15)} & 81.45 (0.29) & 76.58 (0.08) & \textbf{87.89 (0.45)} & 68.63 (0.40) & 50.04 (3.88) & \textbf{83.60 (0.40)}\\
\median~\cite{yin2018byzantine} & 69.38 (0.58) & 48.39 (2.41) & \textbf{83.95 (0.31)} & 45.95 (3.05) & 27.52 (3.97) & \textbf{68.20 (0.63)} & 27.85 (10.7) & 14.29 (6.23) & \textbf{52.22 (3.73)}\\
\tm~\cite{yin2018byzantine} & 85.98 (0.29) & 87.81 (0.14) & \textbf{89.57 (0.18)} & 79.98 (0.47) & 72.40 (0.49) & \textbf{87.47 (0.12)} & 66.69 (0.47) & 41.32 (4.75) & \textbf{81.72 (0.44)}\\
\clippedclustering~\cite{li2023experimental} & 85.76 (0.16) & 87.86 (0.19) & \textbf{89.47 (0.20)} & 82.25 (0.25) & 73.23 (1.23) & \textbf{87.94 (0.36)} & 73.19 (0.98) & 41.52 (5.63) & \textbf{83.06 (0.62)}\\
			\hline
		\end{tabular}
	\end{adjustbox}
	\end{center}
	\label{momentum}
\end{table*}


\begin{figure*}[ht]
	\begin{subfigure}[b]{\linewidth}
		\centering
		\includegraphics[width=\linewidth]{./figs/cifar10_noniid}
% 			\caption{\fedavg}
\end{subfigure}
    \caption{Impact of various degrees of Non-IID on the robustness of aggregation schemes against ALIE attack. A lower $\alpha$ value indicates a higher degree of Non-IID.}
	\label{atk_noniid}
\end{figure*}

\begin{figure*}[ht]
	\begin{subfigure}[b]{\linewidth}
		\centering
		\includegraphics[width=\linewidth]{./figs/fashion_dp}
% 			\caption{\fedavg}
\end{subfigure}
    \caption{Impact of various DP levels on the robustness of aggregation schemes against ALIE attack. A lower $\epsilon$ value indicates a lower budget for DP. All aggregation rules become more vulnerable to adversarial attacks with a lower privacy budget.}
	\label{atk_dp}
\end{figure*}

\subsubsection{The Risk of Gradient Explosion} 
\label{sec_gradient_explosion}
Another interesting observation in Fig.~\ref{atk_sim} is that four robust aggregation rules fail to handle Noise attacks on Fashion MNIST even when only 10\% of the clients are malicious. Upon closer examination of the gradients and loss values, we observe significant gradient explosions among the benign clients, which prevent the model from converging to the optimal solution. We believe that the decline in performance is attributed not only to substantial deviations but also to the potential detrimental impact of gradient explosions caused by malicious attacks.

In order to validate our findings, we employ two measures to mitigate gradient explosions, i.e., gradient clipping and batch normalization, and show the comparison in Fig.~\ref{gradient_explosion}. When no measures are taken, the training loss shows sudden spikes and ends up with a large value, indicating that the model is unable to converge to an appropriate solution. With gradient clipping and batch normalization, the training process becomes more stable. Batch normalization not only prevents gradient explosions but also accelerates the training process, facilitating faster convergence.
\vspace*{-.5em}
\begin{mybox}
\paragraphb{(Takeaway)} 
Malicious updates could increase the vulnerability of global models to gradient explosions. Consequently, it is imperative to apply effective mechanisms (e.g., clipping and batch normalization) to address this issue. 
\end{mybox}

% Not only does batch normalization prevent gradient explosion, but it also accelerates the training process, allowing for faster convergence

\subsubsection{Impact of Momentum} 
%As an example, we train a lightweight Compact Convolutional Transformers (CCT) network~\cite{hassani2021escaping} on the CIFAR10 dataset~\cite{krizhevsky2009learning} to simulate the attack and defense scenarios.
% 	\tv{why do you choose this model? If there is no particular reason you can just say "as an example".}
% The attack and defense experiment include 60 clients, of which 5 of them are Byzantine clients.
% We randomly split the training set into 20 subsets and allocated them to the 20 clients, of which 5 are Byzantine clients.
% As we suggested in Section~\ref{additional_defense}, momentum is regarded as an additional technique enhancing the robustness of Byzantine-resilient FL. We now examine its effectiveness by training a ResNet on CIFAR10 with ALIE attack. The results are shown in Table~\ref{momentum}. Surprisingly, the integration of server momentum shows minimal improvement in enhancing the robustness of the robust aggregation rules In extremely limited scenarios, whilst it results in even lower accuracy in other scenarios. Comparatively, show consistent improvement of all examined aggregation rules.

As indicated in Section~\ref{additional_defense}, momentum is considered a supplementary technique aiming at bolstering the robustness of Byzantine-resilient FL. In order to evaluate its effectiveness, we conduct experiments by training a ResNet on CIFAR10 under the ALIE attack. The obtained results are presented in Table~\ref{momentum}. Surprisingly, the integration of server momentum demonstrates minimal enhancement in the robustness of the aggregation rules, particularly in extremely limited scenarios, while yielding even lower accuracy in other scenarios. In contrast, the aggregation rules consistently exhibit significant improvements when client momentum is employed.

\vspace*{-.2em}
\begin{mybox}
\paragraphb{(Takeaway)} 
When employed as an auxiliary technique, client momentum confers advantages in defending against ALIE attacks, whereas server momentum tends to exacerbate the vulnerability.
\end{mybox}

\subsubsection{Impact of the degree of Non-IID in datasets}
Figure~\ref{atk_noniid} illustrates the test accuracy results of the ALIE attack on CIFAR10, varying the levels of Non-IID partitioning. It can be observed that the effectiveness of the attack increases significantly when the dataset is highly non-IID  (e.g., $\alpha=0.1$). This observation is consistent with prior studies~\cite{fang2020local,shejwalkar2021manipulating,li2023experimental}. A commonly proposed explanation is that as the local data distributions become significantly different, the model updates diversify, thereby posing an additional challenge for the aggregation rules to perform a proper aggregation.
\vspace*{-.3em}
\begin{mybox}
\paragraphb{(Takeaway)} 
The presence of diverse local data distributions poses a greater challenge for robust aggregation. 
\end{mybox}


\subsubsection{Impact of noise-adding for DP}
Next, we assess the influence of introducing Gaussian noise for DP on the resilience of defenses utilizing Fashion MNIST. Figure~\ref{atk_dp} illustrates that as the privacy budget diminishes, the test accuracy across all aggregation rules declines more rapidly as the number of malicious increases. With a high budget (e.g., $\epsilon = 100.0$), all aggregation rules result in comparable accuracy levels to those without the incorporation of DP noise. In contrast, when the privacy parameter $\epsilon$ equals 1.0, the aggregation rules yield extremely low accuracy (nearly the same as random guessing) when $10\%$  of the clients are malicious.
\vspace*{-.3em}
\begin{mybox}
\paragraphb{(Takeaway)} 
A low budget for DP limits the robustness of robust aggregation rules. This suggests the need for careful consideration and trade-offs between the demands of DP and Byzantine resilience in the practice of FL.
\end{mybox}

==> tables/includes.tex <==
\usepackage{nicefrac}
\usepackage{microtype}
% \usepackage[tableposition=top]{caption}
\usepackage{subcaption}
\usepackage{comment}
\usepackage[switch]{lineno}
\usepackage{thmtools, thm-restate}
\usepackage{times}
\usepackage{wrapfig,lipsum,booktabs}
\usepackage{amsmath,bm}
\usepackage{xspace}
\usepackage{adjustbox}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{bbding}
\usepackage{siunitx}
\usepackage{colortbl}
\usepackage{arydshln}
\usepackage{fancyhdr}
\usepackage{tabularx}
\usepackage{array}
\usepackage{listings}
% \usepackage[hidelinks]{hyperref}
\usepackage{url}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[outline]{contour}
\usepackage{soul}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[flushleft]{threeparttable} % http://ctan.org/pkg/threeparttable
\usepackage{tcolorbox}

\newtcolorbox{mybox}{colback=black!5!white,colframe=black,bottomrule=.25mm,toprule=.25mm,leftrule=.25mm,rightrule=.25mm,left=.25mm,right=.25mm,top=-.25mm,bottom=-.25mm}

\newcommand{\myparatight}[1]{\smallskip\noindent{\bf {#1}:}~}

\hypersetup{colorlinks,urlcolor=blue,citecolor=blue,breaklinks=true}

\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\newcommand{\noaistats}[1]{}  %

\definecolor{darkgreen}{rgb}{0,0.4,0.0}
\definecolor{darkblue}{rgb}{0,0.1,0.3}
\definecolor{darkred}{rgb}{0.7,0.0,0.0}


%New colors defined below
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

%Code listing style named "mystyle"
\lstdefinestyle{mystyle}{
  backgroundcolor=\color{backcolour},   commentstyle=\color{codegreen},
  keywordstyle=\color{magenta},
  numberstyle=\tiny\color{codegray},
  stringstyle=\color{codepurple},
  basicstyle=\ttfamily\footnotesize,
  breakatwhitespace=false,
  xleftmargin=\parindent,
  breaklines=true,
  captionpos=b,
  keepspaces=true,
  numbers=left,
  frame=single,
  numbersep=5pt,
  showspaces=false,
  showstringspaces=false,
  showtabs=false,
  tabsize=2
}

\lstset{style=mystyle}

\newcommand{\paragraphb}[1]{\noindent{\bf #1} }
\newcommand{\all}{\infty}
\newcommand{\lbs}{\ensuremath{B}}
\newcommand{\lepochs}{\ensuremath{E}}
\newcommand{\clientfrac}{\ensuremath{C}}
\newcommand{\loss}{\ell}
\newcommand{\risk}{\mathcal{L}}
\newcommand{\uniform}{\overline{\mathcal{U}}}
\newcommand{\hstar}{{h}^{\ast}}
\newcommand{\SUB}[1]{\ENSURE \hspace{-0.15in} \textbf{#1}}
\newcommand{\algfont}[1]{\textit{#1}}
\newcommand{\aggfont}[1]{\texttt{#1}}
\renewcommand{\algorithmicensure}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\newcommand{\eqdef}{\overset{\text{def}}{=}}
\newcommand{\T}{\rule{0pt}{2.2ex}}
\newcommand{\hatw}{\bm{\hat{w}}}
\newcommand{\barw}{\bm{\bar{w}}}
\newcommand{\barv}{\bm{\bar{v}}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bz}{{\boldsymbol{z}}}
\newcommand{\tildez}{\bm{\widetilde{z}}}
\newcommand{\ba}{\bm{\alpha}}
\newcommand{\bv}{\bm{v}}
\newcommand{\update}{\bm{\Delta}}
\newcommand{\tildew}{\bm{\widetilde{w}}}
\newcommand{\tildef}{{\widetilde{F}}}
\newcommand{\hatv}{\bm{\hat{v}}}
\newcommand{\nc}{K}
\newcommand{\pp}{\mathcal{P}}
\newlength{\pw}
\newcommand{\tildeba}{\widetilde{\bm{\alpha}}}
\newcommand{\tildea}{\widetilde{{\alpha}}}
\newcommand{\ie}{\mathcal{I}_{E}}
\newcommand{\BO}{\mathcal{O}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\qqand}{\qquad \text{and} \qquad}
\newcommand{\qqwhere}{\qquad \text{where} \qquad}
\newcommand{\qqwith}{\qquad \text{with} \qquad}
\DeclareMathOperator*{\E}{\mathbb{E}}
\newcommand{\grad}{\triangledown}
\newcommand{\h}{\frac{1}{2}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand \expect {\mathbb{E}}
\newcommand{\fedavg}{\algfont{FedAvg}\xspace}
\newcommand{\fedsgd}{\algfont{FedSGD}\xspace}
\newcommand{\syncsgd}{\algfont{sync-SGD}\xspace}
\newcommand{\Fedgm}{\algfont{RFA}\xspace}
\newcommand{\ours}{\aggfont{Blades}\xspace}
\newcommand{\clustering}{\aggfont{Clustering}\xspace}
\newcommand{\gm}{\aggfont{GeoMed}\xspace}
\newcommand{\mean}{\aggfont{Mean}\xspace}
\newcommand{\median}{\aggfont{Median}\xspace}
\newcommand{\cc}{\aggfont{CC}\xspace}
\newcommand{\krum}{\aggfont{Krum}\xspace}
\newcommand{\tm}{\aggfont{TrimmedMean}\xspace}
\newcommand{\autogm}{\aggfont{AutoGM}\xspace}
\newcommand{\dnc}{\aggfont{DnC}\xspace}
\newcommand{\clippedclustering}{\aggfont{ClippedClustering}\xspace}
\newcommand{\signguard}{\aggfont{SignGuard}\xspace}
\newcommand{\code}[1]{{\texttt{\color[rgb]{0.03,0,1}{#1}}}}
\newcommand{\tv}[1]{\footnote{{\bf Thiemo: #1}}}


==> tables/pipeline.tex <==
\subsection{A Generic Pipeline}
% \subsection{Unifying Byzantine Fault-Tolerant Distributed SGD with FL}
\label{subsec_fedavg}


Additionally, it is possible to extend \fedavg-family algorithms by incorporating a broader range of operations at both the server and client levels. These additional operations can encompass various aspects of the federated learning process, such as Noise-adding for differential privacy (DP)~\cite{dwork2008differential}, trusted data validation~\cite{cao2021fltrust}, and adaptive learning strategies~\cite{reddi2020adaptive,munoz2019byzantine}. This extension goes beyond the traditional tasks of gradient updating and aggregation, which has implications for the robustness of FL against attacks.

To address these diverse aspects, we propose a unified framework at a high level for studying the challenges associated with Byzantine attacks and defenses in federated learning, encompassing elements such as robust aggregation, local updates, communication efficiency, privacy preservation, and adaptive strategies. This framework would serve as a foundation for researching the challenges related to Byzantine attacks and defenses in FL and inspire us to design and develop a benchmark suite specifically tailored for studying this problem.

==> tables/pipeline_bk.tex <==
\subsection{A Generic Pipeline}
% \subsection{Unifying Byzantine Fault-Tolerant Distributed SGD with FL}
\label{subsec_fedavg}
Prior to the growing concern about Byzantine-resilient FL, the literature has already presented various directions toward making distributed machine learning robust against Byzantine or compromised nodes. The major branch of techniques utilizes robust aggregators to replace the average aggregation rule. When used within its operating assumptions, classic schemes, including~\gm~\cite{chen2017distributed}, \krum~\cite{blanchard2017machine}, \tm~\cite{yin2018byzantine}, and \median~\cite{yin2018byzantine}, guarantee convergence even in an adversarial setting. Notably, the convergence guarantee only applies to distributed SGD, where the parameter aggregates the local gradients reported by the working machines and performs a gradient descent step.


In contrast to traditional distributed SGD, \fedavg-family algorithms differentiate themselves by performing multiple local SGD steps at the client level, aiming to enhance communication efficiency~\cite{mcmahan2017communication}. However, these \fedavg-family algorithms sometimes incorporate the aforementioned robust aggregation rules~\cite{li2023experimental}, which were initially proposed for distributed SGD. Hence, there is a need to integrate and conduct unified research and comparison between the two approaches to explore their combined potential, considering the utilization of local updates in \fedavg-family algorithms and the application of robust aggregation rules derived from distributed SGD.

Additionally, it is possible to extend \fedavg-family algorithms by incorporating a broader range of operations at both the server and client levels. These additional operations can encompass various aspects of the federated learning process, such as Noise-adding for differential privacy (DP)~\cite{dwork2008differential}, trusted data validation~\cite{cao2021fltrust}, and adaptive learning strategies~\cite{reddi2020adaptive,munoz2019byzantine}. This extension goes beyond the traditional tasks of gradient updating and aggregation, which in turn, has implications for the robustness of FL against attacks.

To address these diverse aspects, we propose a unified framework at a high level for studying the challenges associated with Byzantine attacks and defenses in federated learning, encompassing elements such as robust aggregation, local updates, communication efficiency, privacy preservation, and adaptive strategies. This framework would serve as a foundation for researching the challenges related to Byzantine attacks and defenses in FL and inspire us to design and develop a benchmark suite specifically tailored for studying this problem.

==> tables/related_work.tex <==
% \section{Related Work}



